Automatic Inference of Symbolic Permissions for Sequential Java Programs

In mainstream programming languages such as Java, a common way to enable concurrency is to manually introduce explicit concurrency constructs such as multi-threading. In multi-threaded programs, managing synchronization between threads is a complicated and challenging task for the programmers due to thread interleaving and heap interference that leads to problems such as deadlocks, data races. With these considerations in mind, access permission-based dependencies have been investigated as an alternative approach to verify the correctness of multi-threaded programs and to exploit the implicit concurrency present in sequential programs without using explicit concurrency constraints. However, significant annotation overhead can arise from manually adding permission-based specifications in a source program, diminishing the effectiveness of existing permission-based approaches. In this paper,we present a framework, Sip4J, to automatically extract access permission-based implicit dependencies from sequential Java programs, by performing inter-procedural static analysis of the source code. Moreover, we integrate and extend an existing permission-based verification tool, Pulse, to automatically verify correctness of the inferred specifications and to reason about their concurrent behaviors. Our evaluation on some widely-used benchmarks gives strong evidence of the correctness of the inferred annotations and their effectiveness in enabling concurrency in sequential programs.

==> GAPrules.tex <==
%!TEX root = ./permissions.tex
\section{\textbf{\gap syntactical rules for graph construction and permission inference}}\label{app:rules}
\ref{CR} shows the context rules that models the read, write behavior of other methods on the reference object (\var or \localrefvar).
\ref{GR} shows the syntactic rules to construct a permission graph model based on expressions encountered and the referenced (global) objects (\var) in it. The syntactical rules for expressions manipulating the local references (\localrefvar), alias of global objects are shown in \ref{LR}. The notation \lvar represent a local variable declared in a method other than \localrefvar. The syntactical rules for method calls expressions are given in \ref{MC} and \ref{PI} describe the access permission inference rules for \var.

\subsection{
\textbf{Context rules}}\label{CR}
{\small\[
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{\var}\,
\using{\textsf{\textbf{(Context-R, \var)}}}
\justifies
\begin{array}{l}
\,\texttt{addReadEdge(context,\var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var}\,
\using{\textsf{\textbf{(Context-RW, \var)}}}
\justifies
\begin{array}{l}
\,\texttt{addReadEdge(context,\var), addWriteEdge(context,\var)}\, \\\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var}\,
\using{\textsf{\textbf{(Context-N, \var)}}}
\justifies
\begin{array}{l}
\,\texttt{removeReadEdge(\context,\var), removeWriteEdge(\context, \var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvar}\,
\using{\textsf{\textbf{(Context-R, \localrefvar)}}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\var)$\implies$apply(Context-R,\var))}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvar}\,
\using{\textsf{\textbf{(Context-RW, \localrefvar)}}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\var)$\implies$apply(Context-RW,\var))}\, \\\\
\end{array}
\end{prooftree}
\\
\begin{prooftree}
\,\texttt{\localrefvar}\,
\using{\textsf{\textbf{(Context-N, \localrefvar)}}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\var)$\implies$apply(Context-N,\var))}\, \\
\end{array}
\end{prooftree}
\end{tabular}
\]}
\subsection{\textbf{Rules for global references}}\label{GR}

{
\small
\[\centering
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{<Type> \var}\,
\using{\textsf{(\textbf{GR-Decl, \var})}}
\justifies
\begin{array}{l}
\,\texttt{<do-nothing>}\,\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var}\,
\using{\textsf{(\textbf{GR-Read-Only,\var})}}
\justifies
\begin{array}{l}
\,\texttt{addReadEdge(\foo,\var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{[Type] \var = <LITERAL>|\varnum{1}}\,
\using{\textsf{(\textbf{GR-Val-Flow,\var})}}
\justifies
\begin{array}{l}
\,\texttt{addWriteEdge(\foo, \var)($\forall a \in$ aliasOf(\var) addWriteEdge(\foo, a)),(apply(GR-Read-Only,\varnum{1})}\,\\\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{[<Type>] \var = new <Type>(\varnum{2})|<Number\_Literal>}\,
\using{\textsf{(\textbf{GR-New-Obj, \var})}}
\justifies
\begin{array}{l}
\,\texttt{addWriteEdge(\foo,\var),apply(Context-N,\var),(apply(GR-Read-Only,\varnum{2})}\,\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var = \varnum{1}}\,
\using{\textsf{(\textbf{GR-Add-Flow, \var})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\var,\varnum{2})$\implies$removeAliasEdge(\var,\varnum{2})),addAliasEdge(\var,\varnum{1})}\,\\
\,\texttt{apply(GR-Read-Only,\varnum{1})}\,\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{[<Type>] \var = \localrefvar}\,
\using{\textsf{(\textbf{GR-Addr-Flow, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\varnum{1})$\implies$addAliasEdge(\var,\localrefvar))}\, \\\\
\,\texttt{($\exists$aliasEdge(\var,\varnum{2})$\implies$removeAliasEdge(\var,\varnum{2})),apply(GR-Read-Only, \varnum{1})}\,
\end{array}
\end{prooftree}
\end{tabular}
\]
}
{
\small
\[\centering
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{[<Type>] \var = \lvar}\,
\using{\textsf{(\textbf{GR-Addr-Flow,\lvar}})}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\var,\varnum{1})$\implies$removeAliasEdge(\var,\varnum{1})),addAliasEdge(\var,\lvar),}\,\\
%\,\texttt{($\forall$ a $\in$ aliasOf(\var),removeAliasEdge(a,\var))}\,
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{<Type> \var = <Null\_Literal>|MCall(<post-perm>,\varnum{1})}\,
\using{\textsf{(\textbf{GR-NullAddr-Init, \var})}}
\justifies
\begin{array}{l}
\,\texttt{<do-nothing>|MCall(<post-perm>,\varnum{1})}\,
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var = <Null\_Literal>|MCall(<post-perm>,\varnum{2})}\,
\using{\textsf{{(\textbf{GR-NullAddr-Flow, \var})}}}
\justifies
\begin{array}{l}
\,\texttt{addWriteEdge(\foo, \var)($\exists$aliasEdge(\var, \varnum{1})$\implies$removeAliasEdge(\var, \varnum{1}))}\, \\\\
\,\texttt{apply(Context-N, \var),($\forall$ a $\in$ aliasOf(\var),apply(<GR-NullAddr-Flow>, a)))\,}\\
\,\texttt{,apply(MCall(<post-perm>,\varnum{1}))}\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var = \localrefvar}\,
\using{\textsf{(\textbf{GR-SelfAddr-Flow, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar, \var)$\implies$<do-nothing>)}\,\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\var = \var}\,
\using{\textsf{(\textbf{GR-SelfAddr-Flow, \var})}}
\justifies
\begin{array}{l}
\,\texttt{<do-nothing>}\,
\end{array}
\end{prooftree}
\end{tabular}
\]}
\subsection{\textbf{Rules for local reference}}\label{LR}

{\small\[
\centering
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{\localrefvar}\,
\using{\textsf{(\textbf{LR-Read-Only, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar, \var)$\implies$(apply(GR-Read-Only(\var))}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvar = <Number\_Literal>}\,
\using{\textsf{(\textbf{LR-Val-Flow, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar, \var)$\implies$apply(GR-Val-Flow, \var))}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{[<Type>] \localrefvar = \var}\,
\using{\textsf{{(\textbf{LR-Addr-Flow, \var})}}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar, \varnum{1}),removeAliasEdge(\localrefvar,\varnum{1}),addAliasEdge(\localrefvar,\var))}\, \\\\
\,\texttt{apply(GR-Read-Only, \var)}\,
\end{array}
\end{prooftree}
%\\\\
%\begin{prooftree}
%\,\texttt{[<Type>] \localrefvar = \localrefvarnum{1}}\,
%\using{\textsf{(\textbf{LR-Addr-Flow, \localrefvar}})}
%\justifies
%\begin{array}{l}
%\,\texttt{($\exists$aliasEdge(\localrefvar,\var)$\implies$removeAliasEdge(\localrefvar,\var)),}\,\\\\
%\,\texttt{($\exists$aliasEdge(\localrefvarnum{1},\varnum{1})$\implies$addAliasEdge(\localrefvar,\localrefvarnum{1}),apply(GR-Read-Only, \varnum{1}))}\,
%\end{array}
%\end{prooftree}
%\\\\
%\begin{prooftree}
%\,\texttt{\localrefvar = \lvar}\,
%\using{\textsf{(\textbf{LR-Addr-Flow, \lvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{($\exists$aliasEdge(\localrefvar, \var)$\implies$removeAliasEdge(\localrefvar,\var))addAliasEdge(\localrefvar,\lvar),}\, \\
%%\,\texttt{($\forall$ a $\in$ aliasOf(\localrefvar),removeAliasEdge(a,\localrefvar))})\,
%\end{array}
%\end{prooftree}
%\\\\\\
%\begin{prooftree}
%\,\texttt{\localrefvar = new <Type>(\varnum{2}|\localrefvarnum{1}|<Number\_Literal>)||MCall(<post-perm>,\varnum{3})}\,
%\using{\textsf{(\textbf{LR-New-Obj, \localrefvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{($\exists$aliasEdge(\localrefvar,\varnum{1})$\implies$removeAliasEdge(\localrefvar,\varnum{1})}\,\\\\
%\,\texttt{(apply(GR-Read-Only,\varnum{2})|apply(LR-Read-Only, \localrefvarnum{1})|apply(MCall(<post-perm>,\varnum{3})))}\,
%\end{array}
%\end{prooftree}
%\\\\
%\begin{prooftree}
%\,\texttt{\localrefvar = <Null\_Literal>}\,
%\using{\textsf{(\textbf{LR-NullAddr-Flow, \localrefvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{($\exists$aliasEdge(\localrefvarnum{1}, \var)$\implies$removeAliasEdge(\localrefvar, \var),apply(GR-NullAdd-Flow(\var)))}\, \\\\
%\end{array}
%\end{prooftree}
%\\\\
%\begin{prooftree}
%\,\texttt{<Type> \localrefvar = <Null\_Literal>|MCall(<post-perm>,\var)}\,
%\using{\textsf{(\textbf{LR-NullAddr-Init, \localrefvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>)|MCall(<post-perm>,\var)}\,
%\end{array}
%\end{prooftree}
%\\\\
%\begin{prooftree}
%\,\texttt{\localrefvar = \var}\,
%\using{\textsf{(\textbf{LR-SelfAddr-Flow, \localrefvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{($\exists$aliasEdge(\localrefvar,\var) $\implies$ <do-nothing>}\,\\
%\end{array}
%\end{prooftree}
%\\\\
%\begin{prooftree}
%\,\texttt{\localrefvarnum{1} = \localrefvarnum{1}}\,
%\using{\textsf{(\textbf{LR-SelfAddr-Flow, \localrefvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>}\,\\
%\end{array}
%\end{prooftree}
\end{tabular}
\]
}
{\small\[
\centering
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{[<Type>] \localrefvar = \localrefvarnum{1}}\,
\using{\textsf{(\textbf{LR-Addr-Flow, \localrefvar}})}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\var)$\implies$removeAliasEdge(\localrefvar,\var)),}\,\\\\
\,\texttt{($\exists$aliasEdge(\localrefvarnum{1},\varnum{1})$\implies$addAliasEdge(\localrefvar,\localrefvarnum{1}),apply(GR-Read-Only, \varnum{1}))}\,
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvar = \lvar}\,
\using{\textsf{(\textbf{LR-Addr-Flow, \lvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar, \var)$\implies$removeAliasEdge(\localrefvar,\var))addAliasEdge(\localrefvar,\lvar),}\, \\
%\,\texttt{($\forall$ a $\in$ aliasOf(\localrefvar),removeAliasEdge(a,\localrefvar))})\,
\end{array}
\end{prooftree}
\\\\\\
\begin{prooftree}
\,\texttt{\localrefvar = new <Type>(\varnum{2}|<Number\_Literal>}\,
\using{\textsf{(\textbf{LR-New-Obj, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\varnum{1})$\implies$removeAliasEdge(\localrefvar,\varnum{1})}\,\\\\
\,\texttt{(apply(GR-Read-Only,\varnum{2}))}\,
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvar = <Null\_Literal>|MCall(<post-perm>,\var)}\,
\using{\textsf{(\textbf{LR-NullAddr-Flow, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar, \var)$\implies$removeAliasEdge(\localrefvar, \var),}\, \\\\
\,\texttt{($\forall$ a $\in$ aliasOf(\localrefvar),apply(<GR-NullAddr-Flow>, a)),apply(MCall(<post-perm>,\var))\,
}\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{<Type> \localrefvar = <Null\_Literal>|MCall(<post-perm>,\var)}\,
\using{\textsf{(\textbf{LR-NullAddr-Init, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{<do-nothing>)|MCall(<post-perm>,\var)}\,
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvar = \var}\,
\using{\textsf{(\textbf{LR-SelfAddr-Flow, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{($\exists$aliasEdge(\localrefvar,\var) $\implies$ <do-nothing>}\,\\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{\localrefvarnum{1} = \localrefvarnum{1}}\,
\using{\textsf{(\textbf{LR-SelfAddr-Flow, \localrefvar})}}
\justifies
\begin{array}{l}
\,\texttt{<do-nothing>}\,\\
\end{array}
\end{prooftree}
\end{tabular}
\]
}
%\end{minipage}}
%--\subsubsection{\textbf{Local variable rules}}
%\vspace{-5pt}
%\captionof{table}{Local variables rules}
%\fbox{\begin{minipage}{32em}
%{\footnotesize
%\[
%\centering
%\begin{tabular}{l l}
%\begin{prooftree}
%\,\texttt{[<PRIM\_TYPE>] \lvar}\,
%\using{\textsf{{(\textbf{L-Decl, \lvar})}}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>}\, \\
%\end{array}
%\end{prooftree}
%\\\\
%\bigskip
%\begin{prooftree}
%\,\texttt{\lvar}\,
%\using{\textsf{(\textbf{L-Read-Only, \lvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>}\, \\
%\end{array}
%\end{prooftree}
%\\\\
%\bigskip
%\begin{prooftree}
%\,\texttt{[<PRIM\_TYPE>] \lvar = <Number\_Literal>}\,
%\using{\textsf{{(\textbf{L-Val-Init,\lvar})}}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>)}\,
%\end{array}
%\end{prooftree}
%%\\\\
%%\bigskip
%%\begin{prooftree}
%%\,\texttt{<Type> \lvar = MCall(<post-perm>, \var) }\,
%%\using{\textsf{{(\textbf{L-Val-Init,\lvar})}}}
%%\justifies
%%\begin{array}{l}
%%\,\texttt{apply(MCall(<post-perm>, \var))}\,
%%\end{array}
%%\end{prooftree}
%\\\\
%\bigskip
%\begin{prooftree}
%\,\texttt{<REF\_Type> \lvar = \lvarnum{1}}\,
%\using{\textsf{(\textbf{L-Add-Init,\lvar})}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>}\,
%\end{array}
%\end{prooftree}
%%\\\\
%%\bigskip
%%\begin{prooftree}
%%\,\texttt{<Type> \lvar = MCall(<post-perm>, \var)}\,
%%\using{\textsf{(\textbf{L-Add-Init},\lvar})}
%%\justifies
%%\begin{array}{l}
%%\,\texttt{apply(MCall(<post-perm>, \var))}\,
%%\end{array}
%%\end{prooftree}
%%\\\\
%%\bigskip
%%\begin{prooftree}
%%\,\texttt{<Type> \lvar = new <REF\_TYPE>(<Number\_Literal>|\var|\localrefvar)}\,
%%\using{\textsf{(\textbf{L-New-Obj}, \lvar})}
%%\justifies
%%\begin{array}{l}
%%\,\texttt{\textcolor[rgb]{1.00,0.00,0.00}{apply(GR-Read-Only, \var)|apply(LR-Read-Only, \localrefvar)}}\,\\
%%\end{array}
%%\end{prooftree}
%\\\\
%\bigskip
%\begin{prooftree}
%\,\texttt{<REF\_TYPE> \lvar = <Null\_Number\_Literal>}\,
%\using{\textsf{{(\textbf{L-NullAdd-Init,\lvar})}}}
%\justifies
%\begin{array}{l}
%\,\texttt{<do-nothing>)}\,
%\end{array}
%\end{prooftree}
%\end{tabular}
%\]}
%\end{minipage}}
\subsection{\textbf{Method call rules}}\label{MC}
{
\small
\[
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{MCall(<Immutable>, \var)}\,
\using{\textsf{\textbf{MCall(Immutable)})}}
\justifies
\begin{array}{l}
\,\texttt{addReadEdge(\var,\foo) apply(Context-R, \var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{MCall(<Pure>, \var)}\,
\using{\textsf{\textbf{MCall(Pure)})}}
\justifies
\begin{array}{l}
\,\texttt{addReadEdge(\foo,\var), apply(Context-RW, \var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{MCall(<Full>, \var)}\,
\using{\textsf{\textbf{MCall(Full)}}}
\justifies
\begin{array}{l}
\,\texttt{addWriteEdge(\foo,\var), apply(Context-R, \var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{MCall(<Share>, \var)}\,
\using{\textsf{\textbf{MCall(Share)}}}
\justifies
\begin{array}{l}
\,\texttt{addWriteEdge(\foo,\var) apply(Context-RW, \var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{MCall(<Unique>, \var)}\,
\using{\textsf{\textbf{MCall(Unique)}}}
\justifies
\begin{array}{l}
\,\texttt{addWriteEdge(\foo,\var), apply(Context-N, \var)}\, \\
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{MCall(<None>, \var)}\,
\using{\textsf{\textbf{MCall(None})}}
\justifies
\begin{array}{l}
\,\texttt{<do-nothing>}\, \\
\end{array}
\end{prooftree}
\end{tabular}
\]}
%\end{minipage}}
\subsection{\textbf{Access permission inference rules}}\label{PI}


This section shows the graph traversal rules to generate acces permissions on the referenced object (\var).\\

{\small\[
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{$\neg$$\exists$readEdge(context,\var) $\wedge$ $\neg$$\exists$writeEdge(context,\var) $\wedge$ $\exists$readEdge(\foo,\var) $\wedge$ $\exists$writeEdge(\foo,\var)}\,
\using{\textsf{(\textbf{Unique})}}
\justifies
\begin{array}{l}
\,\texttt{unique(\var)}\,
\end{array}
\end{prooftree}
\\\\
\begin{prooftree}
\,\texttt{$\neg$$\exists$writeEdge(\foo,\var) $\wedge$ $\exists$readEdge(\foo, var) $\wedge$ $\neg$$\exists$writeEdge(context,\var) $\wedge$ $\exists$readEdge(context, \var)}\,
\using{\textsf{(\textbf{Immutable})}}
\justifies
\begin{array}{l}
\,\texttt{immutable(\var)} \,
\end{array}
\end{prooftree}
\end{tabular}
\]}
{\small
\[
\begin{tabular}{l l}
\begin{prooftree}
\,\texttt{$\exists$readWriteEdge(\foo,\var) $\wedge$ $\neg$$\exists$writeEdge(context,\var) $\wedge$ $\exists$readEdge(context, \var)}\,
\using{\textsf{(\textbf{Full})}}
\justifies
\begin{array}{l}
\,\texttt{full(\var)} \,
\end{array}
\end{prooftree}
\\\\
\bigskip
\begin{prooftree}
\,\texttt{$\exists$writeEdge(\foo,\var) $\wedge$ $\exists$readEdge(\foo, \var) $\wedge$ $\exists$writeEdge(context,\var) $\wedge$ $\exists$readEdge( context, \var)}\,
\using{\textsf{(\textbf{Share})}}
\justifies
\begin{array}{l}
\,\texttt{share(\var)} \,
\end{array}
\end{prooftree}
\\\\
\bigskip
\begin{prooftree}
\,\texttt{$\neg$$\exists$writeEdge(\foo, \var) $\wedge$ $\exists$readEdge(context, \var) $\wedge$ $\exists$writeEdge(context, \var)}\,
\using{\textsf{(\textbf{Pure})}}
\justifies
\begin{array}{l}
\,\texttt{pure(\var)}\,
\end{array}
\end{prooftree}
\\\\
\bigskip
\begin{prooftree}
\,\texttt{$\neg\exists$writeEdge(\foo, \var) $\wedge \exists$readEdge(\foo, \var) $\wedge \neg\exists$writeEdge(context,\var) $\wedge \neg\exists$readEdge(context, \var)}\,
\using{\textsf{(\textbf{None})}}
\justifies
\begin{array}{l}
\,\texttt{None(\var)}\,
\end{array}
\end{prooftree}
\\\\
\bigskip
\begin{prooftree}
\,\texttt{$\neg\exists$writeEdge(\foo, \var) $\wedge \neg\exists$readEdge(\foo, \var) $\wedge \neg\exists$writeEdge(context,\var) $\wedge \neg\exists$readEdge(context, \var)}\,
\using{\textsf{(\textbf{None})}}
\justifies
\begin{array}{l}
\,\texttt{None(\var)}\,
\end{array}
\end{prooftree}
\end{tabular}
\]}

==> algo.tex <==
\newcommand{\DEFAULT}{\mbox{ \bfseries default do}}
\begin{algorithm}\label{infer-algorithm}
%\begin{algorithm}\label{detailed-algorithm}
\SetKwFunction{parsemethod}{\textbf{function:} \textsc{parse-Method}}
\Indm\nonl\parsemethod{$m$}\\
\Indp
\KwIn{$m$}
\KwOut{Anno(($RV(m)$)}
$m \leftarrow$ \textsc{fetchDeclaration}($m$)\;
$sign \leftarrow$ \textsc{parseSignature}($m$)\;
\Set{S} $\leftarrow$ \textsc{fetchStatments}($m$)\;
\ForEach{$s \in$ \Set{S}}{
 \Set{RV}($m$) $\leftarrow$ \textsc{parse-MStatements}($m$, $s$)\;
 }
$mg \leftarrow$ \textsc{construct-Graph}(\Set{RV}($m$))\label{ln:GR}\;
Anno(\Set{RV}($m$)) $\leftarrow$ \textsc{traverseGraph}($mg$)\label{ln:TR}\;
\KwRet{Anno(\Set{RV}($m$))}
\end{algorithm}

\begin{function}[h!]\label{parse-statements}
\SetKwFunction{parsestatement}{function: \textsc{parse-MStatements}
\Indm\nonl\parsestatement{$m,s$}\\
\Indp

\KwIn{$m, s$}
\KwOut{\Set{RV}($m$)}
$es \leftarrow$ \textsc{fetchExpStatement}($s$) \tcp*[l]{\code{fetch expression statement from AST}}
$exp\_type \leftarrow \textsc{fetchExpType}(es)$\tcp*[l]{\code{fetch expression type}}
\Switch{$exp\_type$}{
\hspace{-10pt}\Case{$exp\_type \in ROE$}{
\hspace{-10pt}\Set{RV}($m$) $\leftarrow$ \textsc{parse-ReadOnly-Exp}($es$)\tcp*[l]{\code{parse <read-only> expressions}}
}
\hspace{-10pt}\Case{$exp\_type \in MCE$}{
\hspace{-10pt}\Set{RV}($m$) $\leftarrow$ \textsc{parse-MCall-Exp}($es$)\tcp*[l]{\code{parse method call}}
%\ForEach{rv $\in$ \Set{RV}}{
%\hspace{-10pt}\Set{RV}($m$) $\leftarrow$ \textsc{MethodCall}\code{(<post-perm>, $rv$)}\tcp*[l]{\code{apply <method-call> rules}}
%}
}
\hspace{-10pt}\Case{$exp\_type \in AE$}{
\hspace{-10pt} \Set{RV}($m$) $\leftarrow$ \textsc{parse-Assign-Exp}($es$)\tcp*[l]{\code{parse <read-write> expressions}}}
\hspace{-10pt}\Other{
\hspace{-10pt}\tcp*[l]{\code{recursively parse expression to find the required expression type}}
    }
\hspace{-10pt} \DEFAULT \hspace{5pt} \newline \tcp*[l]{\code{expression type not found}}

\KwRet{\Set{RV}($m$)}
}
}
\end{function}

\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{FMain}{parseReadOnlyExp($Exp\_Type$, $es$)}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{\textnormal{\code{$exp\_Type$, $es$}}}}{
\hspace{-10pt}$v\_bind \leftarrow \textsc{fetchVarBinding}(es)$\;
\hspace{-10pt}$rv \leftarrow \textsc{parseVarExp}(v\_bind)$\;
\hspace{-15pt}\textsc{apply-Rule}(\code{<GR\_READ\_ONLY>},\code{<LR\_READ\_ONLY>},\code{<L\_READ\_ONLY>,$rv$})
\label{ln:applyRule}\tcp*[l]{\code{apply <read-only> graph rule}}
%\caption{parserReadOnlyExp($Exp\_Type$, $e$)}
%\label{proc:parseReadOnly}
}
\end{function}

\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{FMain}{parseMCall($Exp\_Type$, $es$)}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{\textnormal{\code{$Exp\_Type$, $es$}}}}{
\hspace{-10pt}$sub\_m \leftarrow fetchMethod(es)$\tcp*{fetch sub-method}
\hspace{-10pt}\Set{RV}($sub\_m$) $\leftarrow$ \textsc{parse}-Method($sub\_m$)\tcp*[l]{\code{parse sub method}}
\hspace{-10pt}\ForEach{rv $\in$ \Set{RV}}{
\hspace{-15pt}\Set{RV}($m$) $\leftarrow$  \textsc{apply-Rule}(\code{MethodCall}(<post-perm>, $rv$))\tcp*[l]{\code{apply <method-call> rule}}
\hspace{-15pt}\KwRet{\Set{RV}($m$)}
}
}
\end{function}

\begin{function}[h!]\label{fn:constructGraph}
\DontPrintSemicolon
\SetKwFunction{applyRule}{\textsc{apply}-Rule}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\applyRule{\textnormal{\code{GR\_rule}, \code{LR\_rule}, \code{L\_rule}},$var$}}{
  \If{$var$ is \var}{
    $mg \gets$ apply(\code{GR\_rule}, $var$)
  }\ElseIf{$var$ is \localrefvar}{
     $mg \gets$ apply(\code{LR\_rule}, $var$)
  }\ElseIf{$var$ is \lvar}{
    $mg \gets$ apply(\code{L\_rule}, $var$)
  }
  \KwRet $mg$\;
}
\end{function}
\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{parseassignment}{\textsc{parse-Assign}-Exp}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\parseassignment{$e$}}{
\hspace{-10pt}\code{NOC} $\gets \{\code{<CLASS\_INSTANCE\_CREATION>}, \code{<ARRAY\_CREATION>} \}$\label{ln:NOC}\;
\hspace{-10pt}\code{<NULL\_L>} $\gets \{\code{<NULL\_LITERAL>}\}$\label{ln:NAFE}\;
\hspace{-10pt}$le \leftarrow$ \textsc{fetchLHS}($e$)\tcp*[r]{\code{fetch left hand side expression}}
\hspace{-10pt}$re \leftarrow$ \textsc{fetchRHS}($e$)\tcp*[r]{\code{fetch right hand side expression}}
\hspace{-15pt}\If{$le \neq re$}{
\hspace{-15pt}$rexp\_type \leftarrow \textsc{fetchExpType}(re)$\;
\hspace{-15pt}\Switch{$rexp\_type$}{
\hspace{-20pt}\Case{$rexp\_type \in$ \Set{ROE}}{
\hspace{-20pt}\code{$<Type>$} $\leftarrow$ \textsc{fetchDataType}($re$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-LHS-Exp}($le$,\code{$<Type>$})\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-ReadOnly-Exp}($e$, $rexp\_type$)\;
}
\hspace{-20pt}\Case{$rexp\_type \in$ \Set{MCE}}{
\hspace{-20pt}\code{$Type$} $\leftarrow$ \textsc{extractDataType}($re$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-LHS-Exp}($le$,\code{$<Type>$})\;
\hspace{-20pt}\Set{RV} $\leftarrow$ \textsc{parse-Method}($re$)\;
\hspace{-20pt}\ForEach{rv $\in$ \Set{RV}}{
\hspace{-20pt}$mg \leftarrow$ \textsc{MethodCall}\code{(<post-perm>, $rv$)}
}
}
\hspace{-20pt}\Case{\Set{NOC}}{
\hspace{-20pt}$rv \leftarrow$ \textsc{parseRefVars}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-NEW-OBJ>},\newline\code{<LR-NEW-OBJ>}, \code{<L-NEW-OBJ>}, $rv$)
%--\hspace{-20pt}\textsc{\parsereadExp}($rexp\_type$,$re$);
}
\hspace{-20pt}\Case{\code{<NULL\_L>}}{
\hspace{-20pt}$rv \leftarrow \textsc{parseRefVars}(le)$\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-NULL-ADDR-FLOW>},\newline\code{<LR-NULL-ADDR-FLOW>},\code{<L-NULL-ADDR-FLOW>},$rv$)
}
\hspace{-20pt}\Other {
\tcp*[l]{\code{recursively parse right hand side}}
}}}%if ends here
\hspace{-15pt}\ElseIf{$le == re$}{
\hspace{-20pt}$rv \leftarrow$ \textsc{parseRefVars}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-SELF-ADDR-FLOW>},\newline\code{<LR-SELF-ADDR-FLOW>},\code{<L-SELF-ADDR-FLOW>}, $rv$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-ReadOnly-Exp}($re$, $rexp\_type$)
}
\hspace{-15pt}\KwRet $mg$
}
\end{function}
\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{parseLHS}{\textsc{parse}-LHS-Exp}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\parseLHS{\code{$le$,$<Type>$}}}{
\code{<REF\_T>} $\gets \{\code{<REFERENCE\_TYPE>}\}$\label{ln:AFE}\;
\code{<PRIM\_T>} $\gets \{\code{<PRIMITIVE\_TYPE>}\}$\label{ln:VFE}\;
\hspace{-15pt}\Switch{\code{$Type$}}{
\hspace{-20pt}\Case{\code{<PRIM\_T>}}{
\hspace{-20pt}$rv \leftarrow$ \textsc{fetchRefVar}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{apply-Rule}(\code{<GR-VAL-FLOW>},\newline\code{<LR-VAL-FLOW>}, \code{<L-VAL-FLOW>}, $rv$)
}%-- case ends here
\hspace{-20pt}\Case{\code{<REF\_T>}}{
\hspace{-20pt}$rv \leftarrow$ \textsc{fetchRefVar}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{apply-Rule}(\code{<GR-ADDR-FLOW>},\newline\code{<LR-ADDR-FLOW>},\code{<L-ADDR-FLOW>},$rv$)
}% case ends hete
}
\hspace{-15pt}\KwRet $mg$
}
\end{function}

\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{FMain}{parseVarExp($v\_Exp)$)}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{\textnormal{\code{$v\_Exp$}}}}{
\Switch{$v\_Exp$}{
\Case{FIELD}{
$rv \leftarrow fetchRefVar(v\_Exp)$\;
        %apply(\code{<GR-READ-ONLY>}, $rv$)\;
        % \ForEach{$rv \in \mathcal{RV}$}{
        %   $rv \leftarrow \textbf{extractRefVarData}(e)$\;
        %   \todo[inline]{The above isn't clear: $rv$ in the loop head isn't used...}
        % }
}
\Case{PARAMETER}{
$p \leftarrow fetchFormalParams(v\_Exp)$\;
$rv  \leftarrow mapwithGlobalRef(p)$\;\label{proc:parseParam}
        %$\mathcal{VAR}  \leftarrow \textbf{extractRefVar}(p)$\;
        %\ForEach{$var \in \mathcal{VAR}$}{
         %  \code{constructGraph}(\code{<GR-READ-ONLY>}, \code{<LR-READ-ONLY>}, \code{<L-READ-ONLY>}, $var$)\;\label{ln:testapply}
        %}
}
\Case{LOCAL}{\tcp*[f]{if variable is a method's local variable}
$rv \leftarrow mapwithGlobalRef(v\_Exp)$\;
         %\code{constructGraph}(\code{<GR-READ-ONLY>}, \code{<LR-READ-ONLY>}, \code{<L-READ-ONLY>}, $var$)\;\label{ln:testapply}
}

\KwRet $rv$\;
}
}
%\caption{mapGRef($v\_Exp$)}\label{proc:mapGRef}
\end{function}



==> algorithm.tex <==
%!TEX root = ./permissions.tex

\begin{algorithm}[H]
\DontPrintSemicolon
\SetAlgoLined
\caption{The permission inference algorithm.}\label{alg:infer}
\KwIn{\Set{C}, $\{C_1, C_2,\ldots, C_n\}$ the set of classes in the input program}
\KwIn{\Set{M}, $\{M_1, M_2,\ldots, M_n\}$ the set of sets of methods $M_i$, each for a class $C_i$ in $\Set{C}$ }
\KwIn{\Set{CR} $\leftarrow$ $\{Context-Rules\}$}
\KwIn{\Set{SR} $\leftarrow$ $\{Statement-Rules\}$}
\KwIn{\Set{MR} $\leftarrow$ $\{MethodCall-Rules\}$}
\KwIn{\Set{GCR}$\leftarrow$ $CR$ $\cup$ $SR$ $\cup$ $MR$}
\ForEach{m $\in$ $M_i$}{
    \tcc{stage 1}
       \textbf{parseMethod}(\textit{m}){\;
       \qquad $\Set{\foo} \leftarrow$  \textbf{fetchName(m)}\;
       \qquad $\Set{RV} \leftarrow$  \textbf{fetchRefFields(m)}\;
       \qquad $\Set{P} \leftarrow$ \textbf{fetchParams(m)}\;
       \qquad $\Set S \leftarrow $\textbf{fetchStatements(m)}()
       }
       \BlankLine
        \tcc{stage 2}
        $\Set{RVP} \leftarrow $ \textbf{createSetRVP}($\Set{RV}$ $\cup$ $\Set{P}$) \;
        $\Set{Z}   \leftarrow $ \textbf{createSetZ}($\Set{RVP}$ $\cup$ $\{\foo, \context\}$) such that\;
        \qquad \Set{Z} = $\{\var_1, \ldots, \var_n\}$ $\cup$ $\{\param_1, \ldots, \param_n\}$ $\cup$ \{\foo, \context\}

    \BlankLine
    \tcc{stage 3}
    \ForEach{a $\in\Set{Z}$}{
        \textbf{CreateGraphNodes}(\textit{a})  \tcp*{refer to (Section \ref{Gnotations})}
        \qquad\textbf{match}(\textit{a}) \;
        \qquad \Switch{\textit{a}}{
            \qquad \lCase{$\forall{\textit{a}} \in \Set{RVP}$}{
               \qquad createReferenceNodes(\textit{a})
            }
           \Other{
                \qquad createMethodNodes(\textit{a})
           }
    }
}

    \BlankLine
    \tcc{stage 4}
    \ForEach{r $\in\Set{RVP}$}{
        addReadEdge(\foo, \textit{r}, ``r") \tcp* {Assuming that every referenced object (\var) of set \Set{Z} is to be read by the current method \foo.}
    }

    \BlankLine
    \tcc{stage 5}
     \ForEach{rv $\in\Set{RVP}$}{
            \refcontext $\leftarrow$ \textbf{findRefContext}(\textit{rv})\;
        \textbf{match}(\refcontext) \tcp* {refer to (Section \ref{GCR})}
        \Switch{\refcontext}{
            \lCase{R}{
            \;
            \qquad addReadEdge(rv, \context, ``r'')
            }
            \lCase{W}{
                \;
            \qquad addReadEdge(rv, \context, ``r'')\;
            \qquad addWriteEdge(\context, rv, ``w'')
            }
            \lCase{N}{
                \;
            \qquad (do-nothing)
            }
        }
    }

}
\end{algorithm}
\newpage
\begin{algorithm}[H]
\DontPrintSemicolon
\SetAlgoLined
\caption{The permission inference algorithm.}\label{alg:infer1}
\ForEach{m $\in$ $M_i$}{
\BlankLine
    \tcc{stage 6}
    \ForEach{s $\in$ S}{
        \textbf{parseStatements}(\textit{s})\;
        \qquad $expS$ $\leftarrow$ \textbf{findExpType}(\textit{s})\;
        \qquad $GR$ $\leftarrow$ \textbf{matchGRule}($expS$, $\Set{GCR}$) \;
        \qquad $GRD$ $\leftarrow$ \textbf{getRuleDesc}($GR$, $\Set{GCR}$)


        \textbf{match}($GR$)\; \tcp*{needs to discuss}
        \textbf{match}($expS$)\;
        \Switch{$expS$}{
            \lCase{FieldAccess}{\;
            \qquad $GR$ $\leftarrow$ \textbf{matchGRule}($expS$, $\Set{GCR}$)\;
            \qquad $GRD$ $\leftarrow$ \textbf{getGRDesc}($GR$, $\Set{GCR}$)\;
            \qquad $\Set{SRV} \leftarrow$  \textbf{getRefFields}($expS$)\;
             \ForEach{rv $\in$ \Set{SRV}}{
                \qquad ConstructGraph($GRD$, \textit{rv}, \foo, \context)\;
                \qquad addReadEdge(rv, \foo, ``r'')\;
             }
            }
            %--\textbf{match}($expS$) \tcp* {refer to (Section \ref{GCR})}
            \lCase{Assignment}{
                \;

            \qquad $LRV$ $\leftarrow$  \textbf{getLHS}($expS$)\;
            \qquad $\Set{RRV}$ $\leftarrow$  \textbf{getRHS}($expS$)\;
            %--\qquad $GR$ $\leftarrow$ \textbf{matchGRule}($expS$, $\Set{GCR}$)\;
            \qquad addWriteEdge(\foo, $LRV$, ``w'')\;
            \ForEach{rv $\in$ \Set{RRV}}{
                \qquad addReadEdge(\textit{rv}, \foo, ``r'')\;
             }
            }
            %--\textbf{match}($expS$) \tcp* {refer to (Section \ref{GCR})}
            \lCase{VF}{
                \;
            \qquad addWriteEdge(\context, r, ``w'')
            }
            \lCase{NO}{
                \;
            \qquad (do-nothing)
            }
        }
            \ForEach{rv $\in$ \Set{SRV}}{
                \textbf{constructGraph}($GRD$, \textit{rv}) \tcp*{refer to (Section \ref{TR}).
            }
        }
    }

    \BlankLine
    \tcc{stage 7}
    \textbf{TraverseGraph}(\textit{\foo-g})\;
    \ForEach{rv $\in$ \Set{RVP}}{
        $vn$   $\leftarrow$   \textbf{getRefNode}(\foo-g, \textit{rv})
        $\Set{E}$ $\leftarrow$  \textbf{getEdges}($vn$, Direction.OUT, "r")
    }
    \ForEach{e $\in$ \Set{E}}{
          $\Set{MN}$ $\leftarrow$ \textbf{getMethodNode}(e, Direction.IN)
    }
    \ForEach{mn $\in$ \Set{MN}}{
    \textbf{match}($mn$)\;
    \Switch{$mn$}{
      \lCase{\foo}{
                \;
            \qquad (do-nothing)
         }
      }
    }
        %--\textbf{GeneratePermissions}($<$Permission-Inference-Rules$>$, \textit{a})\tcp*{refer to (Section \ref{TR}).}
}
\end{algorithm}




==> analysis-revisited.tex <==
\section{Analysis revisited}

Talk about this.

we try to be as precise as possible. Therefore we
want to minimize the number of false positives: permissions to locations that in reality are
not accessed by the program

==> conclusion.tex <==
\section{Implications}\label{implications}
Access permissions can be used to verify a program behaviour ranging from simple non-null properties to the absence of deadlocks and mutual exclusion to a critical section. 

The automatic inference of permission-based specifications can help programmers to work at a higher level of abstraction letting them focus on the functional and behavioural correctness of the program. It can be used to identify some of the syntactical errors in the program such as \emph{null-pointer} references without compiling the program. This situation can arise in two ways: (a) program error: reference to an object that is a null reference and, (b) permission error: no method generates \code{unique} permission on the referenced object as post-permission. 

For example, in Listing \ref{lst:sa-specprog}, all the methods accessing the shared object, say \code{array1}, would cause null-pointer exception and would remain unsatisfied, if the client program (constructor method) does not instantiate object of \code{array1}, generating the \code{Unique} permission before using it. Similarly, the post-permissions (\code{none(array1)} and \code{none(coll)} of method \code{tidyupColl()} indicates that the object \code{array1} and \code{array2} should be instantiated again, once the method \code{tidyupColl()} has been executed, for these objects to be used by other methods without generating the null-pointer exception. 

Our framework helps programmers automatically identify such errors (if any) in such subtle specifications.
The automatic inference of permission contracts can help automatically compute the dependencies between methods by making the side effects explicit. For example, a close examination of pre-permission of method \code{tidyupColl()} in Listing \ref{lst:sa-specprog} in line 31 shows that the method can only be called if the objects \code{array1} and \code{array2} has \code{Unique} permission as pre-permissions which means it can either be called immediately after the constructor methods \code{ArrayCollection()} and \code{ObjectClass()} as both generate its required permission i.e. \code{unique}, or once all the methods accessing the \code{array1} and \code{array2} object have completed their execution and \code{Unique} permission on the referenced objects have been resumed to be used by other methods. As access permissions pose their own ordering constraints, permission-based dependencies can be used to automatically infer the locking and ordering constraints from the source code of an imperative (sequential) program and parallelise execution of a sequential program for the main-stream programming languages such as \java, to the extent permitted by the computed dependencies, without using any new programming paradigm and run-time to support permissions. Moreover, permission-based parallelisation can free the programmers from the low-level synchronization and reasoning overhead associated with handling multi-threading in imperative programs. 

Similarly, the inference of permission-based lock specifications (such as acquire and release locks with permission invariants) can be used to verify the behaviour of the applications that have already been written using multi-threading without imposing extra work on programmer side. The general idea is to associate permission information with a program reference (thread) to access a particular memory location and track the permission flow through the system to enforce mutual exclusion mechanisms.

Moreover, our framework \gap automatically generates the permission inference and analysis report that provides the developer a quick, abstract and explicit view of the implicit relations (data flow and alias flow) between objects at the method level. Further, having only permission contracts with the method signatures, one can not only check the potential for concurrency in the program but also analyze its behaviour in terms of code reachability analysis (dead code) without looking at the source code.

%We observe that access permission can naturally reason about the divide and conquer static program analysis and verification without imposing extra work on programmers

\begin{comment}
\begin{description}
\item[-] help programmers to work at a higher-level of abstraction and let them focus on the functional and behavioral correctness of the program.
\item[-] allow automatic generation of documentation, amplifying the testing process, and naturally enable assume/guarantee reasoning for divide and conquer static program analysis and verification.
\item[-] increase program comprehension and describe the behaviour of an application and to (re-)design and (or) to resolve the differences between members of a quality assurance team regarding the expected behaviour of the application.
\item[-] provide a quick and abstract view of the relations (data flow and alias flow) between objects at method level and automatically compute the method-level dependencies that is otherwise hard for programmers to analyze by just looking at the code.
For example, a close examination of pre-permission of method \code{tidyupColl()} in Lisiting \ref{lst:sa-specprog} in line 31 shows that the method can only be called if the referenced objects \code{array1} and \code{array2} has \code{Unique} permission as pre-permissions which means it can only be called immediately after the constructor methods \code{ArrayColl()} and \code{ObjectClass()} as both generate its required permission i.e. \code{unique}, otherwise it can be only be called once all the methods accessing \code{array1} and \code{array2} have completed their execution and \code{Unique} permission on the referenced objects have been resumed.

\item[-] help programmers to identify some of the syntactical errors in the program such as \emph{null-pointer} references without compiling the program. This situation can arise in two ways: (a) program error: reference to an object is a null reference itself and, (b) permission error: no method ( constructor) generates \code{unique} permission on the referenced object as post-permission. 

For example, in Listing \ref{lst:sa-specprog}, all the methods accessing a shared object say \code{array1} would cause null-pointer exception and would remain unsatisfied, if the client program does not instantiate the object and create \code{Unique} permission on the referenced object before using it. Similarly, the post-permissions (\code{none(array1)} and \code{none(coll)} of method \code{tidyupColl()} requires that the referenced objects (\code{array1} and \code{array2}) should be instantiated again to be used by other methods to avoid the null-pointer exception.

Our framework, comprises two tools \gap and \pulse, can help programmers automatically identify such errors (if any) in such subtle specifications.

\item[-] analyze the concurrent behavior of a sequential program by considering methods side-effects. 
%As permission-based specifications impose their own ordering constraints, this information.

We observe that permission-based can be used to infer the locking and ordering constraints and automatically parallelise the execution of a sequential \java program to the extent permitted by the data dependencies. The permission-based automatic parallelization will free the programmers from the low-level synchronization and reasoning overhead associated with handling multi-threading and without a need to learn new permission-based programming languages. 
Our evaluation on computationally intensive \java applications using \pulse and the \plaid infrastructure, further shows the effectiveness of the permission-based specifications in enabling concurrency and achieving performance similar to and sometime faster than the un-annotated sequential version of the same program respectively.
\item[-] reason about the correctness (behavior) of a program in terms code (method) reachability analysis also called method (un)satisfiability. The unsatisfiability of a method in a program can be attributed to two reasons: (a) the pre-condition (\code{requires} clause) of a method itself is wrong, or (b) the post condition (\code{ensures} clause) of some other method accessing (creating) the same object is wrong or missing. For example, in line 15 of Listing~\ref{lst:sa-specprog}, it can be seen that method \code{incrColl()} would remain unsatisfied (unreachable) if the client program does not generate \code{full} or the more restrictive permission such as \code{unique} on the referenced object to satisfy its pre-permission. 

\item[-]  The permission-based lock specifications (such as acquire and release locks with permission information) and state invariants can be used to institute concurrency control and to avoid the common concurrency problems such as race conditions and deadlocks in multi-threaded programs without imposing extra work on programmer side. 
The general idea is to associate permission information with a program reference (thread) to access a particular memory location and track the permission 
flow through the system to enforce mutual exclusion mechanisms.
\end{description}
\end{comment}
\section{Threats to Validity}\label{threats}
\input{limitations.tex}
\input{termination.tex}

%As far as soundness of the approaches that are based on static analysis of the program is concerned, according to \cite{Walter2016AutomaticInterpretation}, \quotes{many static analysis tools are sound, meaning that if they prove a property it is guaranteed to hold; on the other hand if they cannot prove a property it might still hold, since analyzers are typically incomplete.} 

In the context of permissions, the analysis is sound if it generates required (enough) permission for each memory location that a method needs to read or write to during its execution. To validate that permission inference mechanism always generates the required (enough) permissions, the analysis is supported by the pre-defined, mathematically specified rules that capture all possible expression types (constructs) in the \javasl and generate permissions to all the globally shared (read or write) objects in a method. The analysis ensures to minimizing the number of false positives (permissions to objects that are not actually accessed in the method from its global environment or the objects that belong to the method's local environment), by following the same set of syntactical rules. Moreover, our evaluation on extensively used benchmark programs and its validation using \pulse and the \gap itself demonstrates the soundness or at least precision of the proposed technique in inferring the correct required (enough) specifications.

%We computed the number of safe approximations by generating and comparing the inferred annotations with the annotations generated manually by a human. While doing so, we observed that identifying dependencies in a small program can be quite easy for a human. However, as the size and complexity of program grows, it becomes increasingly challenging to precisely identify and track the dependency information and manually add it in the program which indeed creates a need for an automatic tool to identify and annotate programs with such subtle dependencies correctly and in an efficient manner.
%\input{validity.tex}

%\section*{Acknowledgment}
%This research was conducted during PhD under Endeavour Postgraduate Award from the Department of Education and Training, Government of Australia at the Faculty of Information Technology, Monash University, Australia. 

==> detailed-algorithm.tex <==
%!TEX root = ./permissions.tex
\newcommand{\DEFAULT}{\mbox{ \bfseries default do}}
\section*{\textbf{Generating Permission-based Specifications: A high level algorithm}}
\begin{algorithm}\label{detailed-algorithm}
\SetKwFunction{parsestatement}{\textsc{parse}-STATEMENT}
\Indm\nonl\parsestatement{$m,s$}\\
\DontPrintSemicolon
\Indp
\Set{ROE} $\gets \{\code{<FIELD\_ACCESS>}, \code{<QUALIFIED\_NAME>}, \code{<SIMPLE\_NAME>}\}$\label{ln:ROE}\;
\Set{MCE}  $\gets  \{\code{<METHOD\_INVOCATION>},\code{<SUPER\_METHOD\_INVOCATION>},\newline  \code{<CONSTRUCTOR\_INVOCATION>},\code{<SUPER\_CONSTRUCTOR\_INVOCATION>}\}$\;
\Set{AE} $\gets \{\code{<ASSIGNMENT>}\}$\;
$e \leftarrow$ \textsc{extractExpr}($s$) \tcp*[r]{\code{extract expression statement from AST}}
$exp\_type \leftarrow \textsc{extractExpType}(e)$\tcp*[r]{\code{fetch expression type}}
\Switch{$exp\_type$}{
\hspace{-10pt}\Case{$exp\_type \in$ \Set{ROE}}{
  \hspace{-10pt}$mg \leftarrow$ \textsc{parse-ReadOnly-Exp}($e$)\tcp*[r]{\code{parse <read-only> expressions}}
  }
\hspace{-10pt}\Case{$exp\_type \in$ \Set{MCE}}{
\hspace{-10pt}\Set{RV} $\leftarrow$ \textsc{parse-Method}($e$)\tcp*[r]{\code{parse sub method}}
\hspace{-10pt}\ForEach{rv $\in$ \Set{RV}}{
\hspace{-10pt}$mg \leftarrow$ \textsc{MethodCall}\code{(<post-perm>, $rv$)}\tcp*[r]{\code{apply <method-call> rules}}
     }
  }
\hspace{-10pt}\Case{$exp\_type \in$ \Set{AE}}{
\hspace{-10pt}$mg \leftarrow$ \textsc{parse-Assign-Exp}($e$)\tcp*[r]{\code{parse <read-write> expressions}}
  }
\hspace{-10pt}\Other{
\hspace{-10pt}\tcp*[r]{\code{recursively parse expression to find the required expression type}}
    }
\hspace{-10pt}\DEFAULT $\hspace{5pt}$ \newline \tcp*[r]{\code{expression type not found}}

  \KwRet{$mg$}
}
\end{algorithm}
\begin{algorithm}
\caption{Permission Inference Algorithm}
\label{infer-algorithm}
%\begin{algorithm}\label{detailed-algorithm}
\SetKwFunction{parsemethod}{\textsc{parse}-METHOD}
\Indm\nonl\parsemethod{$m$}\\
\DontPrintSemicolon
\Indp
$m \leftarrow$ \textsc{getDeclaration}($m$)\tcp*[r]{\code{fetch method declaration expression}}
 $sign \leftarrow$ \textsc{parseSignature}($m$)\tcp*[r]{\code{parse method signature}}
 \Set{S} $\leftarrow$ \textsc{getStatments}($m$)\tcp*[r]{\code{fetch method statements}}
 \ForEach{$s \in$ \Set{S}}{
 \quad \Set{RV}($m$) $\leftarrow$ \textsc{\parsestatement}($m$, $s$) \tcp*[r]{\code{parse each method statement}}
}
$mg \leftarrow$ \textsc{construct-Graph}\Set{RV}($m$)\label{ln:GR}\tcp*[r]{\code{apply graph construction rules}}
Annotated (\Set{RV}($m$)) $\leftarrow$ \textsc{traverseGraph}($mg$)\label{ln:TR}\tcp*[r]{\code{apply permission inference rules}}
\KwRet Annotated (\Set{RV}($m$)) \tcp*[r]{\code{referenced variables with permissions}}
\end{algorithm}

\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{parsereadExp}{\textsc{parse-READONLY}-Exp}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\parsereadExp{$e$}}{
%\begin{algorithm}
%\SetKwFunction{parsereadExp}{\textsc{parse-READONLY}-Exp}
%\Indm\nonl\parsereadExp{$e,exp-type$}\\
%\Indp
%\DontPrintSemicolon
%--\Switch{$exp\_type$}{
%--\hspace{-10pt}
%--\Case{\code{<FIELD\_ACCESS>} or \code{<QUALIFIED\_NAME>} or \code{<SIMPLE\_NAME>}}{
\hspace{-10pt}\Set{RV} $\gets$ \textsc{extractRefVar}($e$)\label{ln:parseRefVars}\tcp*[r]{\code{extract global referenced variable}}
\hspace{-10pt}\ForEach{rv $\in$ \Set{RV}}{
\hspace{-10pt}$mg \gets$ \textsc{constructGraph}(\code{<GR\_READ\_ONLY>},\code{<LR\_READ\_ONLY>},\code{<L\_READ\_ONLY>,$rv$)}\label{ln:applyRule}\tcp*[l]{\code{apply graph construction rules}}
}
%--\hspace{-10pt}\textsc{traverseGraph}($mg$)\label{ln:TR}\tcp*[r]{apply permission inference rules}
%--}
%\hspace{-10pt}\Case{
%\code{<METHOD\_INVOCATION>} or \code{<CLASS\_INSTANCE\_CREATION>} orW
%\code{<CONSTRUCTOR\_INVOCATION>}  or \code{<SUPER\_METHOD\_INVOCATION>}
%\qquad \quad \code{<SUPER\_CONSTRUCTOR\_INVOCATION>}}
%{
%\hspace{-10pt}$\Set{RV} \leftarrow $ \textsc{parse-Method}($e$) \tcp*[r]{parse sub method}
%\hspace{-10pt}\ForEach{rv $\in$ \Set{RV}}{
%\hspace{-10pt}\textsc{MethodCall}\code{(<post-perm>, $rv$)}\tcp*[r]{apply method call rule to add referenced variables in the caller method}
%}%loop ends here
%}% case ends here
\hspace{-5pt}\KwRet $mg$\;
}
\end{function}
\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{parsemethod}{\textsc{parse-Method}}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\parsemethod{$m$}}{
$_m \leftarrow$ \textsc{getMDeclaration}($m$)\tcp*[r]{\code{fetch method declaration expression}}
$\Set{SIGN} \leftarrow$ \textsc{parseMSignature}($m$)\tcp*[r]{\code{parse method signature}}
\Set{S} $\leftarrow$ \textsc{getMStatments}($m$)\tcp*[r]{\code{fetch method statements}}
\ForEach{$s \in$ \Set{S}}{
  \Set{RV(m)} $\leftarrow$ \textsc{\parsestatement}($m$, $s$) \tcp*[r]{\code{parse each statement}}
}
$\Set{mg} \leftarrow$ \textsc{constructMGraph}($Rv(m)$)\label{ln:GR}\tcp*[r]{\code{apply graph construction rules}}
$\Set{Anno(RV(m))} \leftarrow$ \textsc{traverseMGraph}($mg$)\label{ln:TR}\tcp*[r]{\code{apply permission inference rules}}
\KwRet $\Set{RV}$\tcp*[r]{\code{referenced variables with permissions}}
}
\end{function}
\begin{function}[h!]\label{fn:parsemethod}
\DontPrintSemicolon
\SetKwFunction{constructGraph}{\textsc{construct}-Graph}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\constructGraph{\textnormal{\code{GR\_rule}, \code{LR\_rule}, \code{L\_rule}},$var$}}{
  \If{$var$ is \var}{
    $mg \gets$ apply(\code{GR\_rule}, $var$)
  }\ElseIf{$var$ is \localrefvar}{
     $mg \gets$ apply(\code{LR\_rule}, $var$)
  }\ElseIf{$var$ is \lvar}{
    $mg \gets$ apply(\code{L\_rule}, $var$)
  }
  \KwRet $mg$\;
}
\end{function}
\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{parseassignment}{\textsc{parse-Assign}-Exp}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\parseassignment{$e$}}{
\hspace{-10pt}\code{NOC} $\gets \{\code{<CLASS\_INSTANCE\_CREATION>}, \code{<ARRAY\_CREATION>} \}$\label{ln:NOC}\;
\hspace{-10pt}\code{<NULL\_L>} $\gets \{\code{<NULL\_LITERAL>}\}$\label{ln:NAFE}\;
\hspace{-10pt}$le \leftarrow$ \textsc{extractLHS}($e$)\tcp*[r]{\code{fetch left hand side expression}}
\hspace{-10pt}$re \leftarrow$ \textsc{extractRHS}($e$)\tcp*[r]{\code{fetch right hand side expression}}
\hspace{-15pt}\If{$le \neq re$}{
\hspace{-15pt}$rexp\_type \leftarrow \textsc{extractExpType}(re)$\;
\hspace{-15pt}\Switch{$rexp\_type$}{
\hspace{-20pt}\Case{$rexp\_type \in$ \Set{ROE}}{
\hspace{-20pt}\code{$<Type>$} $\leftarrow$ \textsc{extractDataType}($re$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse}-LHS-Exp($le$,\code{$<Type>$})\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-ReadOnly-Exp}($e$, $rexp\_type$)\;
}
\hspace{-20pt}\Case{$rexp\_type \in$ \Set{MCE}}{
\hspace{-20pt}\code{$Type$} $\leftarrow$ \textsc{extractDataType}($re$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-LHS-Exp}($le$,\code{$<Type>$})\;
\hspace{-20pt}\Set{RV} $\leftarrow$ \textsc{parse-Method}($re$)\;
\hspace{-20pt}\ForEach{rv $\in$ \Set{RV}}{
\hspace{-20pt}$mg \leftarrow$ \textsc{MethodCall}\code{(<post-perm>, $rv$)}
}
}
\hspace{-20pt}\Case{\Set{NOC}}{
\hspace{-20pt}$rv \leftarrow$ \textsc{parseRefVars}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-NEW-OBJ>},\newline\code{<LR-NEW-OBJ>}, \code{<L-NEW-OBJ>}, $rv$)
%--\hspace{-20pt}\textsc{\parsereadExp}($rexp\_type$,$re$);
}
\hspace{-20pt}\Case{\code{<NULL\_L>}}{
\hspace{-20pt}$rv \leftarrow \textsc{parseRefVars}(le)$\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-NULL-ADDR-FLOW>},\newline\code{<LR-NULL-ADDR-FLOW>},\code{<L-NULL-ADDR-FLOW>},$rv$)
}
\hspace{-20pt}\Other {
\tcp*[l]{\code{recursively parse right hand side}}
}}}%if ends here
\hspace{-15pt}\ElseIf{$le == re$}{
\hspace{-20pt}$rv \leftarrow$ \textsc{parseRefVars}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-SELF-ADDR-FLOW>},\newline\code{<LR-SELF-ADDR-FLOW>},\code{<L-SELF-ADDR-FLOW>}, $rv$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{parse-ReadOnly-Exp}($re$, $rexp\_type$)
}
\hspace{-15pt}\KwRet $mg$
}
\end{function}
\begin{function}[h!]
\DontPrintSemicolon
\SetKwFunction{parseLHS}{\textsc{parse}-LHS-Exp}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\parseLHS{\code{$le$,$<Type>$}}}{
\code{<REF\_T>} $\gets \{\code{<REFERENCE\_TYPE>}\}$\label{ln:AFE}\;
\code{<PRIM\_T>} $\gets \{\code{<PRIMITIVE\_TYPE>}\}$\label{ln:VFE}\;
\hspace{-15pt}\Switch{\code{$Type$}}{
\hspace{-20pt}\Case{\code{<PRIM\_T>}}{
\hspace{-20pt}$rv \leftarrow$ \textsc{extractRefVar}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-VAL-FLOW>},\newline\code{<LR-VAL-FLOW>}, \code{<L-VAL-FLOW>}, $rv$)
}%-- case ends here
\hspace{-20pt}\Case{\code{<REF\_T>}}{
\hspace{-20pt}$rv \leftarrow$ \textsc{extractRefVar}($le$)\;
\hspace{-20pt}$mg \leftarrow$ \textsc{construct-Graph}(\code{<GR-ADDR-FLOW>},\newline\code{<LR-ADDR-FLOW>},\code{<L-ADDR-FLOW>},$rv$)
}% case ends hete
}
\hspace{-15pt}\KwRet $mg$
}
\end{function}

%\begin{function}[h!]
%\DontPrintSemicolon
%\SetKwFunction{FMain}{parseVarExp($v\_Exp)$)}
%\SetKwProg{Fn}{Function}{:}{}
%\Fn{\FMain{\textnormal{\code{$v\_Exp$}}}}{
%\Switch{$v\_Exp$}{
%      \Case{FIELD}{
%        $rv \leftarrow \textbf{extractRefVar}(v\_Exp)$\;
%        %apply(\code{<GR-READ-ONLY>}, $rv$)\;
%        % \ForEach{$rv \in \mathcal{RV}$}{
%        %   $rv \leftarrow \textbf{extractRefVarData}(e)$\;
%        %   \todo[inline]{The above isn't clear: $rv$ in the loop head isn't used...}
%        % }
%      }
%      \Case{PARAMETER}{
%        $p \leftarrow \textbf{extractFormalParam}(v\_Exp)$\;
%        $rv  \leftarrow \textbf{mapGRef}(p)$\;\label{proc:parseParam}
%        %$\mathcal{VAR}  \leftarrow \textbf{extractRefVar}(p)$\;
%        %\ForEach{$var \in \mathcal{VAR}$}{
%         %  \code{constructGraph}(\code{<GR-READ-ONLY>}, \code{<LR-READ-ONLY>}, \code{<L-READ-ONLY>}, $var$)\;\label{ln:testapply}
%        %}
%      }
%      \Case{LOCAL}{\tcp*[f]{if variable is a method's local variable}
%        $rv \leftarrow \textbf{mapGRef}(v\_Exp)$\;
%         %\code{constructGraph}(\code{<GR-READ-ONLY>}, \code{<LR-READ-ONLY>}, \code{<L-READ-ONLY>}, $var$)\;\label{ln:testapply}
%      }
%
%      \KwRet $rv$\;
%    }
%}
%\caption{mapGRef($v\_Exp$)}\label{proc:mapGRef}
%\end{function}
%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$c$,$m$}
  % \KwOut{$c$,$m$}
      \quad \textbf{parseMSignature}(\textit{$c$,$m$})\;
      \quad  $\Set{ST} \leftarrow$ \textbf{fetchMStatements}(\textit{$m$})  \;
      \quad \ForEach{s $\in$ $ST_i$}{
            \textbf{parseMStatement}(\textit{$m$,$s$}) \;
       }
\caption{parseMethod(c, m)}\label{proc:parseMethods}
\end{procedure}}
%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$m$}
  % \KwOut{$m$}
    $m-id \leftarrow$ \textbf{fetchMIdentifier}(\textit{$m$})\;
    $m-retType \leftarrow$ \textbf{fetchMReturnType}(\textit{$m$})\;
    $m-mod \leftarrow$ \textbf{fetchMModifier}(\textit{$m$})\;
    $m-id \leftarrow$ createMethod($c$,$m-mod$,$m-id$,$m-retType$)\;
    $\Set{MParams} \leftarrow$ \textbf{fetchMParameters}(\textit{$m$})\;
    \textbf{parseMParamsAsRefFields}(\textit{$m$,$\Set{MParams}$})\;

\caption{parseMSignature(m)}\label{proc:parseMSignature}
\end{procedure}}
%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$m$,$\Set{MParams}$}
  \KwOut{$m$}
    $\Set{THIS-INV} \leftarrow$ \textbf{fetchThisMethInvocation}(\textit{$m$})\;
    \ForEach{p $\in$ $MParams_i$}{
      \ForEach{inv $\in$ $THIS-INV_i$}{
        \quad $\Set{ARGS} \leftarrow$  \textbf{fetchArguments}(\textit{$inv$})\;
         \ForEach{arg $\in$ $ARGS_i$}{
            \If{matchArgwithParam($arg$,$p$)}{
            \tcp*{match position and type of the parameter with the argument}
                    \If{arg.isField}{
                       \qquad ${rv} \leftarrow$ \textbf{extractRefVarData}($arg$)\;
                       \qquad ${p}  \leftarrow$ \textbf{extractParamData}($p$)\;
                       \qquad addRefParam($m$,$p$,$rv$)\;
                       \qquad addRefField($m$,$rv$)\;
                       \qquad apply(<GR-READ-ONLY>, $rv$)\;
                    }
                    \If{arg.isLocal}{
                         \qquad  ${rv} \leftarrow$  \textbf{findpointeeFieldofLocalVariable}($arg$)\;
                         \qquad ${rv} \leftarrow$ \textbf{extractRefVarData}($rv$)\;
                         \qquad ${p}  \leftarrow$ \textbf{extractParamData}($p$)\;
                         \qquad \textbf{addRefParam}($m$,$p$,$rv$)\;
                         \qquad \textbf{addRefField}($m$,$rv$)\;
                         \qquad apply(<GR-READ-ONLY>, $rv$)\;
                    }

                % {
                }

%-----------------
    }
}
}
\caption{parseMParamsAsRefField(m, $\Set{MParams}$) }\label{proc:addMParamsAsRefFields}
\end{procedure}}

%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$m$}
  \KwOut{$\Set{THIS-INV}$}
     \quad \textbf{visitAllCompilationUnits()}\;
     \quad $\Set{M\_INV} \leftarrow$  \textbf{fetchMethodInvocations}()\;
      \quad \ForEach{inv $\in$ $\Set{M\_INV}$}{
       \qquad $\Set{THIS-INV}$ $\leftarrow$ matchThisMInvocation($inv$,$m$);
    }
\caption{fetchThisMethInvocation(m)}\label{proc:fetchThisMethInvocations}
\end{procedure}}

%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$m$, $s$}
  \KwOut{$\Set{RV}$}
  $sType$  $\leftarrow$ \textbf{fetchExpStatype}(\textit{$s$})\;
  \uIf{$sType$ == <FieldAccess> $\lor$ $sType$ == <QualifiedName>}{
    $e$ $\leftarrow$ \textbf{fetchExpression}(\textit{$s$})\;
    $\Set{RV}$ $\leftarrow$  \textbf{parseRefVars}($e$)\;
    \ForEach{rv $\in \Set{RV}$}{
      apply(<GR-READ-ONLY>, $rv$)\;
      addRefField($m$,$rv$)\;
    }
  }
   \uElseIf{$sType$ == <METHODINVOCATION>}{
     $sm$ $\leftarrow\leftarrow$  \textbf{fetchMethodCalls}(\textit{$sm$})\;
     $sm_{id}$ $\leftarrow$  \textbf{parseMethod}(\textit{$sm$})\;
    }
    \uElseIf{$sType$ == <SimpleName>}{
           $e$ $\leftarrow$ \textbf{fetchExpression}(\textit{$s$})\;
           \eIf{e.isField}{
             $\Set{RV}$ $\leftarrow$  \textbf{parseRefVars}($e$)\;
             \ForEach{rv $\in \Set{RV}$}{
                 $rv$ $\leftarrow$  \textbf{extractRefVarData}($e$)\;
                 apply(<GR-READ-ONLY>, $rv$)\;
                 addRefField($m$,$rv$)\;
              }
            }
            {%----
                \eIf{e.isParameter}{
                     $p$  $\leftarrow$ \textbf{extractParamData}($e$)\;
                     \textbf{updateRefParam}($m$,$p$,$rv$)\;
                     $\Set{RV}$ $\leftarrow$  \textbf{parseRefVars}($p$)\;
                     \ForEach{rv $\in$ $\Set{RV}$}{
                         apply(<GR-READ-ONLY>, $rv$)\;
                         \textbf{updateRefField}($m$,$rv$)\;
                     }
                }{%----
                    \If{e.isLocal}{
                        $rv$ $\leftarrow$  \textbf{findpointeeFieldofLocalVariable}($e$)\;
                        $rv$ $\leftarrow$ \textbf{extractRefVarData}($rv$)\;
                        apply(<LR-READ-ONLY>, $rv$)\;
                        \textbf{addRefField}($m$,$rv$)\;
                    }
                }
         }
    }%--- Simple Name ends here
         \uElseIf{$sType$ == <ASSIGNMENT>}{
           $e$ $\leftarrow$ \textbf{fetchExpression}(\textit{$s$})\;
           $le$ $\leftarrow$ \textbf{fetchLHS}(\textit{$e$})\;
           $re$ $\leftarrow$ \textbf{fetchRHS}(\textit{$e$})\;
           \If{$re$ == <PRIMTIVE\_TYPE> $\lor$ $re$ == <LITERAL>}{
                 $\Set{RV} \leftarrow$  \textbf{parseRefVars}($le$)\;
                 \ForEach{rv $\in \Set{RV}$}{
                   apply(<GR-VAL-FLOW>, $rv$) $\lor$ apply(<LR-VALUE-FLOW>,$rv$)\;
                   addRefField($m$,$rv$)\;
                 }
                $\Set{RV} \leftarrow$  \textbf{parseRefVars}($re$)\;
                \ForEach{rv $\in \Set{RV}$}{
                  apply(<GR-READ-ONLY>, $rv$) $\lor$ apply(<LR-READ-ONLY>, $rv$)\;
                  addRefField($m$,$rv$)\;
                }
            }
             \ElseIf{$re$ == <ClassInstanceCreation> $\lor$ $re$ == <ArrayCreation>}{
                 $rv \leftarrow$  \textbf{parseRefVars}($le$)\;
                 apply(<GR-NEW-OBJ>,$rv$) $\lor$ apply(<LR-NEW-OBJ>, $rv$)\;
                 addRefField($m$,$rv$)\;
                 $\Set{RV} \leftarrow$  \textbf{parseRefVars}($re$)\;
                \ForEach{rv $\in \Set{RV}$}{
                  apply(<GR-READ-ONLY>, $rv$) $\lor$ apply(<LR-READ-ONLY>,$rv$)\;
                  addRefField($m$,$rv$)\;

                }
           }
               \ElseIf{$re$ == <REFERENCE\_TYPE>}{
                  $rv \leftarrow$  \textbf{parseRefVars}($le$)\;
                  apply(<GR-ADDR-FLOW>, $rv$) $\lor$ apply(<LR-ADDR-FLOW>, $rv$)\;
                  addRefField($m$,$rv$)\;
                  $\Set{RV} \leftarrow$  \textbf{parseRefVars}($re$)\;
                  \ForEach{rv $\in \Set{RV}$}{
                    apply(<GR-READ-ONLY>, $rv$) $\lor$ apply(<LR-READ-ONLY>, $rv$)\;
                    addRefField($m$,$rv$)\;
                 }
               }
                \ElseIf{$re$ == <NULL\_LITERAL>}{
                  $rv \leftarrow$  \textbf{parseRefVars}($le$)\;
                  apply(<GR-NULL-ADDR-FLOW>, $rv$) $\lor$ apply(<LR-NULL-ADDR-FLOW>, $rv$)\;
                  addRefField($m$,$rv$)\;
                }
                \ElseIf{$re$ == $le$}{
                  apply(<GR-SELF-ADDR-FLOW>, $rv$) $\lor$ apply(<LR-SELF-ADDR-FLOW>, $rv$)\;
                  addRefField($m$,$rv$)\;
                }
    }
\caption{parseStatement(m, s)}\label{proc:parseStatement}
\end{procedure}}

%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$rv$}
  \KwOut{$rv$}
    \quad $rv-name  \leftarrow$ \textbf{fetchRefVarName}(\textit{$rv$})\;
    \quad $rv-type  \leftarrow$ \textbf{fetchRefVarType}(\textit{$rv$})\;
    \quad $rv-class  \leftarrow$ \textbf{fetchRefVarDeclarClass}(\textit{$rv$})\;
    \quad $con-Operation \leftarrow$ \textbf{chooseContext}(\textit{$rv$})\;
    \quad $m-Operation  \leftarrow$ \textbf{fetchMOperations}(\textit{$rv$})\;
    \quad $alias-Operation  \leftarrow $  \textbf{fetchAliaseInfo}(\textit{$rv$})\;
\caption{Extract Referenced Field(s) Data}\label{proc:extractRefVarData}
\end{procedure}}

%%%--- IGNORED PROCEDURE
\ignore{\begin{procedure}
  \KwIn{$rv$}
  \KwOut{$rv$}
     \quad $p-name  \leftarrow$ \textbf{fetchParamName}(\textit{$rv$})\;
    \quad $p-type  \leftarrow$ \textbf{fetchParamType}(\textit{$rv$})\;
    \quad $p-decl-m  \leftarrow$ \textbf{fetchParamDeclarMethod}(\textit{$rv$})\;
   \quad  $con-Operation \leftarrow$ \textbf{chooseContext}(\textit{$rv$})\;
    \quad  $m-Operation  \leftarrow$ \textbf{fetchMOperations}(\textit{$rv$})\;
    \quad  $alias-Operation  \leftarrow$  \textbf{fetchAliaseInfo}(\textit{$rv$})\;
\caption{Extract Parameter(s) Data}\label{proc:extractParamData}
\end{procedure}}

%%%--- IGNORED PROCEDURE
\ignore{\begin{algorithm}[htb]
\DontPrintSemicolon
\SetAlgoLined
\caption{The permission inference algorithm: Graph Construction}\label{alg:infer}
\BlankLine
\KwIn{$\Set{Data}$} \tcp*{ where D is the output data from the parsing module}
\BlankLine
    \tcc{stage 1}
    $\Set{C} \leftarrow$ \textbf{getClasses}(\textit{$\Set{Data}$})   \;
    \BlankLine
    \tcc{stage 2}
        \ForEach{c $\in$ $C_i$} {
            $\Set{M} \leftarrow$ \textbf{getMethods}(\textit{$c$})  \;
            \tcc{stage 3}
             \ForEach{m $\in$ $M_i$}{
                \textbf{createMethodGraph}(\textit{m}){  \tcp*{refer to Graph notations(Section~\ref{Gnotations})}
                  \BlankLine
                    \tcc{Step 1}
                   createMethodNode($\foo$)\;
                   createContextNode($\context$)\;
                   \BlankLine
                    \tcc{Step 2}
                    \ForEach{v $\in$ $\Set{RV}$}{
                       createReferenceNode(\textit{v}) \;
                       \BlankLine
                         \tcc{Step 3}
                         addReadEdge(\foo, v, ``r") \tcp* {Assuming that every referenced object (\var) of set \Set{Z} is to be read by the current method \foo.}\;
                         \BlankLine
                          \tcc{Step 4}
                         $mop \leftarrow$ getMethodOperation(\textit{v})\;
                          \Switch{$mop$}{
                                 \lCase{W}{
                                    \;
                                   addReadEdge(v, \foo, ``r'')\;
                                   addWriteEdge(\foo, v, ``w'')
                                }
                                 \lCase{N}{
                                    \;
                                  (do-nothing)
                                }
                            }
                            \BlankLine
                          \tcc{Step 5}
                         $cop \leftarrow$ getContextOperation(\textit{v}) \;
                         \textbf{match}($cop$) \tcp* {refer to Graph Construction (Section~\ref{GCR})}
                            \Switch{$cop$}{
                                 \lCase{R}{
                                \;
                                addReadEdge(v, \context, ``r'')
                                }
                                 \lCase{W}{
                                    \;
                                addReadEdge(rv, \context, ``r'')\;
                                addWriteEdge(\context, rv, ``w'')
                                }
                                \lCase{N}{
                                    \;
                                (do-nothing)
                                }
                            }
                        }
                      }
               }
            }

\end{algorithm}}

% \newpage

%%%--- IGNORED PROCEDURE
\ignore{\begin{algorithm}[htb]
\DontPrintSemicolon
\SetAlgoLined
\caption{The permission inference algorithm: Permission Generation}\label{alg:infer1}
\todo[inline]{What's the input of this algorithm? The result of graph construction? But since we're parsing individual statements again, it doesn't seem so...}
\ForEach{m $\in$ $M_i$}{
\BlankLine
\tcc{stage 6}
\ForEach{s $\in$ $\Set{S}$}{
    \textbf{parseStatements}(\textit{s})\;
    $expS$ $\leftarrow$ \textbf{findExpType}(\textit{s})\;
    $GR$ $\leftarrow$ \textbf{matchGRule}($expS$, $\Set{GCR}$) \;
    $GRD$ $\leftarrow$ \textbf{getRuleDesc}($GR$, $\Set{GCR}$)\;
    \textcolor[rgb]{1.00,0.00,0.00}{\textbf{match}($GR$)}\;
    \todo[inline]{needs to discuss}
    \textbf{match}($expS$)\;
    \Switch{$expS$}{
        \lCase{FieldAccess}{\;
        $GR$ $\leftarrow$ \textbf{matchGRule}($expS$, $\Set{GCR}$)\;
        $GRD$ $\leftarrow$ \textbf{getGRDesc}($GR$, $\Set{GCR}$)\;
        $\Set{SRV} \leftarrow$  \textbf{getRefFields}($expS$)\;
         \ForEach{rv $\in$ \Set{SRV}}{
            ConstructGraph($GRD$, \textit{rv}, \foo, \context)\;
            addReadEdge(rv, \foo, ``r'')\;
         }
        }
        %--\textbf{match}($expS$) \tcp* {refer to (Section~\ref{GCR})}
        \lCase{Assignment}{
            \;
        $LRV$ $\leftarrow$  \textbf{getLHS}($expS$)\;
        $\Set{RRV}$ $\leftarrow$  \textbf{getRHS}($expS$)\;
        %--$GR$ $\leftarrow$ \textbf{matchGRule}($expS$, $\Set{GCR}$)\;
        addWriteEdge(\foo, $LRV$, ``w'')\;
        \ForEach{rv $\in$ \Set{RRV}}{
            addReadEdge(\textit{rv}, \foo, ``r'')\;
         }
        }
        %--\textbf{match}($expS$) \tcp* {refer to (Section~\ref{GCR})}
        \lCase{VF}{
            \;
        addWriteEdge(\context, r, ``w'')
        }
        \lCase{NO}{
            \;
        (do-nothing)
        }
    }
        \ForEach{rv $\in$ \Set{SRV}}{
            \textbf{}($GRD$, \textit{rv}) \tcp*{refer to (Section~\ref{TR}).
            \todo[inline]{Why are we constructing graph here?}
        }
    }
}
\BlankLine
\tcc{stage 7}
\textbf{TraverseGraph}(\textit{\foo-g})\;
\todo[inline]{Is this shown in the paper?}
\ForEach{rv $\in$ \Set{RVP}}{
    $vn$   $\leftarrow$   \textbf{getRefNode}(\foo-g, \textit{rv})\;
    $\Set{E}$ $\leftarrow$  \textbf{getEdges}($vn$, Direction.OUT, "r")\;
}
\ForEach{e $\in$ \Set{E}}{
      $\Set{MN}$ $\leftarrow$ \textbf{getMethodNode}(e, Direction.IN)
}
\ForEach{mn $\in$ \Set{MN}}{
\textbf{match}($mn$)\;
\Switch{$mn$}{
  \lCase{\foo}{
            \;
        (do-nothing)
     }
  }
}
        %--\textbf{GeneratePermissions}($<$Permission-Inference-Rules$>$, \textit{a})\tcp*{refer to (Section~\ref{TR}).}
}
\end{algorithm}} 

==> limitations.tex <==

We identified some threats to the validity of permission inference technique and the generalizability of our results.

%\begin{description}
%\item[\textbf{Construct Validity}] 

The permission inference framework does not support all the language constructs in \javasl at the moment such as method overriding (polymorphism), generics and lambda expressions. This is because the technique is based on statically analysing the source code. We perform flow-sensitive analysis of the code to determine the actual instance type (the type of the object on the right-hand side) assigned to a reference of base type on the left-hand side. This information can eventually be used to determine which overridden method should be parsed as a result of the method call without actually executing the program. Moreover, our evaluation on a small to large sized benchmark programs shows that through \gap we have provided a succinct methodology to infer access permissions from realistic \java programs implementing rich constructs of \javasl. 

%\item[\textbf{Internal Validity}]
In certain situations, the permission inference technique does not produce optimal (precise) solutions and generate safe (restrictive) permissions i.e., \textsf{unique} or \textsf{full} instead of \textsf{immutable} or \textsf{pure}. This happens when a) an object is accessed in a complex infix expression with nested pre-fix or post-fix expressions or b) an object is accessed in a library method call expression. The first case is because the permission extractor does not individually parse complex infix-postfix expressions and the analysis is based on type of expression such as \code{Field\_Access} and \code{Assignment}  encountered in the AST of program. The second case is due to the unavailability of method definitions (bodies) for the library methods. We believe this is an engineering problem and generating safe/restrictive permissions will not affect the integrity of the program itself when actually used for program verification or parallelization.

%\end{description}
%For example, for the expression \code{Parent p = new Child();}, the proposed technique can determine that reference \code{p} refers to an object of type \code{Child} and for a method call expression \code{p.foo()}, the overridden method from the \emph{Child} class should be parsed. The graph construction and traversal process would be same to handle dynamic method calls and generate permissions on the referenced objects.


==> name.tex <==
It is observed that writing manual specifications in source code is laborious and error-prone job for the programmer. The annotation overhead is one of the reasons that hinders the wider adoption of these approaches. Ideally, it would be much easier and more effective for a programmer to omit or not to be concerned with writing permission-based annotations, while still being able to exploit benefits offered by such annotations. Therefore, in this research work, our aim is to automatically extract permission based specifications from the source code of a \java program.

==> pulse-analysis.tex <==
%!TEX root = ./permissions.tex

\begin{figure}[htb]
\begin{lstlisting}[morekeywords={none,full,unique,ensures,requires,alive,ALIVE,alive,share,immutable,pure,main},
label=lst:a-pluralspecprog,caption={The Pulse translate version of the annotated program given in Listing \ref{lst:sa-specprog}.}]
import edu.cmu.cs.plural.annot.*;
@ClassStates({@State(name = "alive")})

class ArrayCollection{
@Perm(ensures="unique(this) in alive")
ArrayCollection() {   }
@Perm(requires="unique(this) in alive * unique(#0) in alive",
      ensures="unique(this) in alive * unique(#0) in alive")
public void createColl(Integer[] coll) { 
} 
@Perm(requires="pure(this) in alive * pure(#0) in alive",
ensures="pure(this) in alive * pure(#0) in alive")
public void printColl(Integer[] coll) { 
} 
@Perm(requires="pure(this) in alive * pure(#0) in alive",
      ensures="pure(this) in alive * pure(#0) in alive")
public void computeStat(Integer[] coll) { 
} 
@Perm(requires="pure(this) in alive * pure(#0) in alive",
     ensures="pure(this) in alive * pure(#0) in alive")
 boolean isSorted(Integer[] coll) { } 
@Perm(requires="pure(this) in alive * pure(#0) in alive",
     ensures="pure(this) in alive * pure(#0) in alive")
 Integer findMax(Integer[] coll) { } 
@Perm(requires="full(this) in alive * full(#0) in alive",
      ensures="full(this) in alive * full(#0) in alive")
public void incrColl(Integer[] coll) { } 
@Perm(requires="unique(this) in alive * unique(#0) in alive",
ensures="unique(this) in alive * unique(#0) in alive")
public void tidyupColls(Integer[] coll) { } 
}
ENDOFCLASS
@ClassStates({@State(name = "alive")})

class ObjectClass {
@Perm(ensures="unique(this) in alive")
ObjectClass() {   }
@Perm(requires="full(this) in alive * full(#0) in alive * pure(#1) in alive",
    ensures="full(this) in alive * full(#0) in alive * pure(#1) in alive")
void manipulateObjects(Client p1, Client p2) { }
}
ENDOFCLASS
@ClassStates({@State(name = "alive")})
class Client {
@Perm(ensures="unique(this) in alive")
Client() {   }
@Perm(requires="unique(this) in alive",
      ensures="unique(this) in alive")
public static void main(String[] args) { } 
}
ENDOFCLASS
\end{lstlisting}
\end{figure}

==> pulse-translation.tex <==
%!TEX root = ./permissions.tex

\begin{comment}
\pulse performs following analysis as a part of verifying permission-based specifications at method level:
\begin{description}
\item[\textbf{1. Satisfiable methods:}] A method is satisfied if all its pre-conditions are met. The method satisfiability analysis is performed using the \code{requires} clause in the input specifications. It checks whether a method can be reached from another method based on its permission contract.
\item[\textbf{2. Unsatisfiable methods:}] The presence of an unreachable or unsatisfiable method indicates that no possible client can fulfil the method's contract i.e., the \code{requires} clause and this method is not called under any circumstances; thus the method remains unreachable. The presence of the unreachable method is due to the method's unsatisfiable pre-conditions which indicates an error in the inferred specifications.
\item[\textbf{3. Concurrent methods:}] It computes 
the number (percentage) of methods that can be parallelised with at-least one other method or itself based on permission contract. It, therefore, computes the possible concurrency among methods. 
%the set of immutable (independent) methods i.e., methods that never change state of an objects or that does not produce side effects. 
\item[\textbf{4. Sink states:}] the presence of states without successors (sink state) may lead to deadlock.
\item[\textbf{5. Unreachable states:}] the presence of unreachable states arise due to a method's unsatisfiable pre-condition shows an error in the specifications.
%\item[\textbf{6. Typestate Transition Matrix.}] control flow of the program through typestates to verify the expected design of the program.
\end{description}
In our research, we are interesting in exploiting first three analysis made by \pulse as inferring and verifying typestates is not an immediate objective of this research. 
\end{comment}
To reconcile the differences between \gap and \pulse, a number of characteristics of \pulse and \plural are worth noting.
\begin{itemize}
\item Firstly, \plural is a permission-based specification language where access permissions are defined at object level using keyword \ ``\code{this}''. It does not support permission annotations at the field level e.g.\ \code{pure(this.field)} and \code{pure(obj.field)} etc., so is the \pulse. In \gap, we generate permissions at the class field level that can help enable concurrency at a more granular level.

\item Secondly, \pulse tool does not support \textsf{share} and \textsf{immutable} permission as a part of analysis. This is because, referring to the permission coexistence semantics in Table \ref{table:Table1}, \textsf{share} cannot coexist with either \textsf{unique}, \textsf{full} or \textsf{immutable}, and \textsf{immutable} cannot coexist with either \textsf{share} or \textsf{full}. Hence, \pulse's concurrency analysis of methods cannot be performed on these annotations.

\item Thirdly, \pulse follows the \DbC and support permission contract of the form \code{P$\implies$Q} where the relation $P \mbeq Q$ (the pre and post conditions should be same to fulfill the permission contract between caller and the callee method) should hold to maintain integrity of the specifications during analysis but the situation can be different in reality. 

For example, in Listing \ref{lst:sa-specprog} line 30, the permission inference technique generates permission contract for method \code{tidyupColl()} with different pre- and post-permission. This is because as there is a null address flow statement for \code{coll}. In this case, we generate `None' permission as post-permission to show that object \code{coll} is a null reference now and a new instance of the object should be created with \textsf{unique} permission to used it again in the program after the method \code{tidyupColl()} is executed.

\item Fourthly, \pulse does not support overloaded constructors and methods even if the method is provided with different return type, parameters and permission contracts. So, we need to ignore the overloaded constructors (methods) in the \pulse translated version. Moreover, \pulse always requires a non-parameterized (default) constructor to define \textsf{unique} permission on the receiver object (\code{this}) and perform permission analysis for rest of the methods at class level.  
\end{itemize}


==> reasoning-concurrecny-analysis.tex <==
%!TEX root = ./titlepage.tex

\subsection{Pulse Analysis}
As mentioned earlier, we analyse the extracted permissions using \pulse in terms of specification correctness and potential for concurrency, and the results can be found in Figure~\ref{fig:example_pulse}.
\subsubsection{Correctness Analysis of Inferred Specification}
\pulse verifies correctness of inferred permission-based contracts in terms of method satisfiability. 
\begin{description}
\item[\textbf{Method Satisfiability}]:
A method is satisfied if all of its pre-conditions (\texttt{requires} clause) are met, which means that it can be reached from another method. The analysis results show that in the sample example, all the methods are satisfied with their permission contracts that means every method got its required permissions, generated by another method, and is satisfied with its contract which in-turn ensures the absence of unreachable code (method) in the program and validate the correctness of our proposed technique in generating correct permissions.
\item[\textbf{Null-Pointer Analysis}]:
\begin{figure}[h!tb]
\begin{center}
\begin{subfigure}[t]{0.4\textwidth}
\includegraphics[scale=.8]{img/example_sat.pdf}
\caption{Satisfiability of methods.}
\end{subfigure}
\subsubsection{Concurrency Analysis based on Inferred Specifications} 
Further, the analysis of concurrency matrix shows that 7 out of 8 methods can be parallelised based on the permission contracts. It demonstrates the effectiveness of the inferred specifications in extracting concurrency from a sequential program, which is one of the motivations of our work. Detailed evaluation of some benchmark programs is described in the next section.
\begin{subfigure}[t]{0.5\textwidth}
\includegraphics[scale=.8]{img/example_con.pdf}
\caption{Method concurrency matrix.}
\end{subfigure}
\caption{Correctness analysis (left) and potential concurrency analysis (right) of methods of the \code{BoxCollection} class as produced by \pulse.}\label{fig:example_pulse}
\end{center}
\end{figure} 
\end{description}


==> significances.tex <==
\section{Significance of the inferred specifications}
The significance of this work can be attributed as follows:
The inferred permission-based contracts 
 \begin{itemize}
 \item free programmers from the annotation overhead associated for manually adding access notations and other information in the program 
 that otherwise may needs to be added for each invocation of the method and for all input parameters
 \item increase program comprehension by providing a quick and abstract view of the relations (data flow and alias flow) between variables that is otherwise hard for programmers to analyze by just looking at method bodies.
 \item allow automatic generation of documentation, amplifying the testing process, and naturally enable assume/guarantee reasoning for divide and conquer static program analysis and verification.
 \item Specifications
can be used by engineers to generate a collection of documents describing
the behaviour of an application. This documentation can be used by engineers to (re-)design an application or to resolve differences between members of a quality assurance
team regarding the expected behaviour of the application.
\item allows programmers to work at a higher-level of abstraction without generating any intermediate representations and focus on functional properties of a program.
\item help programmers achieve concurrency, without mastering the intricacies of explicit concurrency domain.
\item help programmers by makings implicit dependencies explicit, can be used to avoid side effect (data races) and achieve concurrency, without mastering the intricacies of explicit concurrency domain.
 \item automatically parallelise execution of sequential programs without any extra-work imposed on programmers.
 \item complement existing permission-based verification approaches to formally reason about concurrency without any extra-work needed on programmer's side.
 \item Unlike previous approaches, our technique infers permissions for \java, a mainstream programming language used widely in industry, without the need of any intermediate specifications.
 \item We generate permissions at more granular level that can be used to exploit maximum concurrency present in the program.
 \end{itemize}


==> termination.tex <==
%The correctness of any algorithm is always concerned with a) the soundness of the analysis and(or) if the analysis terminates successfully.

%As far as termination of the proposed algorithm is concerned, the permission extraction mechanism is recursive in nature and termination of recursive algorithms is considered as an undecidable problem in general. 

The termination of our permission inference technique is based on the following characteristics. a) The analysis is based on AST of the source code, a parse tree having a finite number of nodes (sub-expressions) for an expression statement. Therefore, it takes a finite number of steps to parse a finite number of expressions in the generated AST. b) It always converges to an expression type designated as the base case or otherwise terminates the analysis successfully.

The presence of indirect or chained recursion, as explained previously in section \ref{meta-analysis}, can cause indefinite (infinite) loops and consequently the memory overflows. However, we observe and validate using realistic benchmarks that the proposed analysis terminate successfully. This is because we save the meta-data (at-least its signature) of each method and its current state before parsing its body and switching the control to parse sub-method calls in it. This step helps to identify the second level indirect recursive method call, for the same method during parsing and ensure that analysis terminates successfully. 

Another threat for the successful termination can be the \code<self-address-flow> statements (when a reference directly or indirectly starts pointing to itself creating a loop for analysis), the technique identifies such expressions following the appropriate syntactical rules, and terminates successfully without creating any loop or cycles in the graph construction and traversal process eventually.


%For example, during analysis when a reference (direct or indirect) starts pointing to itself, or to a local reference that is not an alias of a global reference or when a reference becomes a null reference, the proposed technique will follow the appropriate syntactic rules such as \code{(GR-SelfAddr-Flow, \var)}\footnote{When expression statement is of the form \var = \var;} and \code{(GR-NullAddr-Flow, \var)}\footnote{when expression statement is of the form \var = null;}, to identify loops, cycles and null references in the underlying program and eventually terminates the graph construction process.
%Therefore, they make graph traversal simple and there is no backtracking in the constructed graph to ensures the termination of analysis and the inference mechanism itself.

==> tool.tex <==
d%!TEX root = ./permissions.tex

\section{Sip4J Implementation}\label{tool}
We implemented an Eclipse Plugin \gap \textcolor[rgb]{1.00,0.00,0.00}{available at ......} Furthermore, we integrated \pulse tool with \gap to demonstrate the correctness of inferred specifications and to demonstrate effectiveness of the inferred specifications. The permission inference technique in \gap consists of three main tasks: (a) AST-based modular analysis, (b) graph construction and (c) graph traversal. Section \ref{modular-analysis} explains the \gap analysis to automatically infer permission-based dependencies at method level.

\subsection{Sip4j Analysis}\label{modular-analysis}
As discussed previously, \gap performs modular static analysis of the source code based on AST following syntactical rules (Section \ref{GCR}) to perform data flow and alias flow analysis of the source code. The extracted information is represented as a graph structure using graph notations (section \ref{Gnotations}, a single graph for each method which is eventually used to automatically reveal permission-based dependencies at method level, using permission inference rules (Section \ref{TR}).

\fbox{Should we remove this paragraph, summary of \gap analysis already given in section \ref{sec:method}}
\textcolor[rgb]{1.00,0.00,0.00}{At the first stage, it generates Abstract Syntax Tree (AST) of the source code to fetch and parse all the compilation unit and set of classes in each compilation unit. For every class, it parses set of methods and for each method, it extracts and stores the data flow, alias flow and context information (access through other methods) for all the referenced variables accessed inside a method body from its global environment. The syntactical rules for analysis are based on the type of expression(s) encountered in AST while parsing method's statements such as \code{<FIELD\_ACCESS>}, \code{<ASSIGNMENT>} or \code{<METHOD\_INVOCATION>} etc,. and the type of referenced variable(s), such as a class field (\var) or a local reference variable (\localrefvar) or a local variable (\lvar) other than \localrefvar accessed in each expression. At the second stage, the extracted information is represented as a graph structure, a single graph for each method using graph notations (section \ref{Gnotations}). The graph structure is eventually used to automatically reveal permission-based dependencies at method level, using permission inference rules (Section \ref{TR}).
}
Starting with an input \java program with a set of compilation units having set of user-defined classes and set of methods in each class. For each \textit{method}, the proposed technique parses a method's signature and its body by fetching \code{<MethodDeclaration>} expression node from the generated AST, in following ways:

\begin{description}
\item[\textbf{Method's Signature:}] In parsing a method's signature, its name, return type, visibility modifier,
formal parameters are all stored in a data structure (\Set{SIGN}) using function \textsc{parse-Signature}(). It is worth mentioning here that the proposed technique maps all the formal parameters with their corresponding arguments (actual parameters) by fetching corresponding method invocations at project level. For each parameter and for each invocation of the method, we analyse whether the actual parameter (argument) is a
global variable (a class field) (\var) or a method's local reference (\localrefvar) that is an alias of a global reference \var or a method's local variable (\lvar) other than \localrefvar. This information is then used to perform dataflow and alias flow analysis of the actual referenced object(s) accessed in a method through parameters and to generate permissions on the actual referenced object. This step ensures integrity of data by tracking changes to the actual objects across multiple methods.
\item[\textbf{Method's Body:}]
The procedure \textsc{parse-Method}() parses a method body. In parsing a method's body, method statements are parsed one by one using procedure \textsc{parse-Statement}() that takes a statement (\code{$s$}) in a method (\code{$m$}). It recursively parses each statement to perform the data flow, alias flow and context analysis of all the referenced variables accessed in each expression in a statement. For this purpose, each expression is parsed based on its expression type. For example, the read-only expressions (\Set{ROE}) are parsed using function \textsc{parse-readOnly-Exp}(), the assignment expressions (\Set{AE}) are parsed using function \textsc{parse-Assign-Exp}() and method calls expressions (\Set{MCE}) are handled using function \textsc{parse-Method}().

During parsing, we extracts and stores all the referenced variables accessed in a method ($m$), along with the data flow, alias flow and context information, in a data structure (\Set{RV}). Further, based the type of referenced variable(s) (\var, \localrefvar, \lvar) accessed in each expression, appropriate syntactical rules are applied to constructs graph structure ($mg$), from the extracted information using function \textsc{construct-Graph}(). The permission inference rules are then applied on each graph ($mg$) (function \textsc{traverse-Graph}) to generate permissions on all the referenced variables (\Set{RV}) accessed at method level.\\\\
During parsing, different expressions are handled in following ways:\\
\begin{itemize}
\item{\textbf{Read-Only Expression(s):}}
The expressions categorized as \Set{ROE} are handled using function \textsc{parse-readOnly-Exp}() that takes an input expression (\code{e}). It parse \code{e} to extract the referenced variable(s)(\Set{RV}) with the required (read) information (function \textsc{extractRefVar()}, line no. \code{\ref{ln:parseRefVars}})). It then applies different versions of graph construction rules such as \code{(GR-READ-ONLY,\var)}, \code{(LR-READ-ONLY,\localrefvar)} etc. using function \textsc{construct-Graph}()(line no. \code{\ref{ln:applyRule}}), depending on the type of referenced variables (\var, \localrefvar, \lvar) accessed in each expression.
\item{\textbf{Assignment Expression(s):}}
The proposed technique performs flow-sensitive analysis of the source program where type of a reference object on left side of an assignment statement is determined based on right hand side expression of this statement. The syntactical rules for an assignment statement are categorized depending on the expression statement type (\code{<NULL\_Literal>} or (\code{<CLASS\_INSTANCE\_CREATION>} etc.) and the data type of right hand side expression such as reference type(\code{<REF\_T>}) or primitive type \code{<PRIM\_T>}. The handling of assignment statements is detailed in a separate function, \textsc{parse-Assign-Exp}() that recursively parses right and left hand side of an assignment statement to determine the type of syntactical rules applicable at any moment.

For example, if a right hand side expression in an assignment statement yields to a reference type (\code{<REF\_T>}), the proposed technique applies address flow rules such as \code{(GR-ADDR-FLOW,\var)}, \code{(LR-ADDR-FLOW, \localrefvar)} or \code{(L-ADDR-FLOW,\lvar)}) rule on the left operand(s) of the assignment statement, whereas in case the right hand side expression yields to a \code{<PRIM\_T>}, the chosen rule can be \code{(GR-VAL-FLOW,\var)} or \code{(LR-VAL-FLOW,\localrefvar)} etc., depending on the type of reference variable accessed. All other expressions are parsed accordingly.
\item{\textbf{Method Invocation Expression (s):}}
The method call rules (Section \ref{methodR}) are used to parse a method invocation expression such as \code{<METHOD\_INVOCATION>}, \code{<CONSTRUCTOR\_INVOCATION>} etc., encountered during parsing.
As a part of modular analysis, the procedure \textsc{parse-Method()} is recursively called for every sub method (called) inside a (caller) method. The analysis of the caller method completes when all of its sub methods (called) have been parsed and permissions on the referenced variables in the called method have been generated.
\begin{itemize}
\item For a non-recursive method call, the proposed technique extracts corresponding method \code({$sub\_m$}) binding using method declaration (\code{<METHOD\_DECLARATION>}) node in AST. Each sub method \code({$sub\_m$}) is parsed, using procedure \textsc{parse-Method}(), to generates permissions on all the referenced variable(s) (\Set{RV}) accessed in it. The proposed technique then applies appropriate method call rule \code{MethodCall(<post-perm>, \var)} to generate permissions for the caller method.
\item The proposed analysis skips the \code{<METHOD\_INVOCATION>} expression for a recursive method call(where a method calls itself). This is because we expect to extract the read and write behavior of a method on the referenced variables and recursive calls does not change the way a method accesses referenced variables as a part of method statements.
\item The constructor calls (\code{CLASS\_INSTANCE\_CREATION}, \code{<SUPER\_CONSTRUCTOR\_INVOCATION>}) are handled the same way as any other non-recursive method call using their corresponding (\code{<METHOD\_DECLARATION>}) node from the AST. For constructor methods, we use either \code{GR-NEW-Obj, \var} or \code{LR-NEW-Obj, \localrefvar} rule that ensures that constructor method always generates \textsf{unique} permissions on referenced object.
\item The super method calls are parsed the same way as other non-recursive method calls by fetching the corresponding (\code{<METHOD\_DECLARATION>}) expression from the parent class but the proposed technique does not handle overridden method calls (when child overrides a method in parent) for the moment and thereby dynamic method dispatch\footnote{In Java, dynamic method dispatch is a mechanism by which a call to an overridden method is resolved at runtime and the version of the overridden method to execute is based on the type of object it refer to}. But it can integrate dynamic method dispatching, based on the expression-based syntactical rules we use for analysis purpose to decide which overridden method should be parsed as a result of overridden method call.

\item Static method dispatching (to multiple targets) is straightforward and that is determined using method's signature and the static type of the receiver object at compile time. For example, for a method call x.foo(10) where x is an instance of class X, we parse \code{foo()} method of class X having an argument type \code{int} or where type of argument is a subtype of its formal parameter type.
       %\begin{lstlisting}[label=lst:u-specprog,caption={The un-annotated \code{BoxColl} class in \java}]
%class Parent{
% public void foo(){
%  System.out.println("Parent foo() called");
% }
%}
%class Child extends Parent{
% public void foo(){
%   System.out.println("Child foo()called");
% }
% public static void main(String[] args){
%   Parent p = new Child();
%   p.foo();  //calls Child's version of foo
% }
%}
%\end{lstlisting}
\item In case of library method calls, we generate safe permissions i.e., \textsf{unique} or \textsf{full} on the referenced object, regardless of the actual read and write behavior that method performs on it. This is because we do not have definition of the library method.
\end{itemize}
\end{itemize}
\end{description}
\input{detailed-algorithm}
\subsubsection{Termination Analysis}
The algorithm for parsing method statements is recursive in nature and the termination of recursive algorithms is an undecidable problem in general. Our proposed technique ensures termination of the analysis performed in following ways:
\begin{itemize}
\item The source code analysis is based on AST, a parse tree having finite number of nodes (sub expressions) for an expression statement. Therefore, source code analysis takes finite number of steps to parse a finite number of expressions in the generated AST.
\item The proposed algorithm is designed in a way that it always converges to a base case characterised by an expression type such as \code{<FIELD\_ACCESS>} or \code{<ASSIGNMENT>} etc at statement level.
\item Further, we skip method invocation expression(s) for recursive call(s) as explained already. In case of infinite recursive calls (when a method \code{foo1()} calls method \code{foo2()} that again calls \code{foo1()}), our analysis terminates successfully. This is because, we maintain a data structure to store the extracted information from a method and the method itself. During parsing, we skip the second level recursive call for method \code{foo1()} in \code{foo2()} as \code{foo1()} is already present in the data structure and continue parsing from the next expression in the caller method \code{foo2()}.
\item Further, syntactical rules for graph construction are developed in such a way that it guarantees no cycle or loop in the constructed graph. Therefore, graph traversal is simple and there is no backtracking in the graph that further ensures termination of analysis and the inference itself.
\end{itemize}


==> validity.tex <==
%!TEX root = ./titlepage.tex

\subsection{Threats to Validity Lesson Learned}

\begin{description}
\item[External Validity]
We may think that we can make certain generalisations from our results, but we cannot say with certainty that this take place. 

This reflects the fact that there are many threats to external validity that can undermine our results,

External validity checks our confidence by asking questions:

 1) Whether the study’s results are applicable to other groups (generalization of the technique and the results)?
 
 2) To what extent can our result/mechanism can be generalised 
    (a) to a wider population, and/or 
    (b) across populations (languages in my case), treatments (technique), settings/contexts, and time?

We want to know if our findings from the sample benchmark programs can be generalised to other unobserved programs in the population.

To assess the extent, we have to determine how well the sample (or population) that we have studied represents the wider population. To have confidence, we would need to ensure that our sample program closely mirrored the population programs; that is, confidence that our sample shared similar characteristics (language (Java), size (Lines of code), constructs (java specification language), complexity (rich constructs)) to the population.

Threats to external validity are any factors within a study that reduce the generalisability (or generality) of the results. 

\begin{itemize}
\item[selection biases] 
No two programs are the same. 
you need to make sure that the groups are equivalent before you start which may explain the differences in scores on the dependent variable. In other words, you need to take into account such individual differences when selecting data for your research.

When the sample that is studied does not represent the population that the researcher hopes to make generalisations to, there has been a selection bias. Where selection bias occurs, it is difficult (or maybe impossible, depending on the level of selection bias) to argue that the results that come from a biased sample can be generalised to the wider population.

Selection bias can be reduced in an experimental design approach bay randomly selecting the samples, which mean that participants in the different groups that are being compared are similar across a range of general and specific characteristics. 

The more general characteristics when randomly assigning participants to different groups include factors such as language and imperative object-oriented  nature of programs. 

A study may only look at certain characteristics of a population; that is, it will not necessarily look for every difference in the relationships studied (usually between two variables) across sample characteristics (e.g., age, gender, attitudes, personality, etc.). However, it may be differences in these sampling characteristics that limit the generalizability of results to a wider population.

\item[The use of other student samples] across the population (some limitations are being caused by \pulse) it will inevitably result in selection bias, reducing the ability to make generalisations to a wider population,

\item[Constructs, methods, and external validity]


\item[Construct Validity]

To make a study construct valid, we have to narrow down broad concepts we may be interested in constructs that can be measured

Single measure -In my case it is concurrency analysis, annotation overhead for a \java program and the execution time of the permission analysis itself
We have to perform some statistical analysis of the results based on a single construct.

In my case, different aspects (different measure) of a construct ( size, complexity) to make generalization Therefore, we have to be careful about making generalisations about the effect of the construct A, background music, on construct B, task performance, because We were making generalisations from our results about background music in general; in other words, all types of background music, and all volumes of background music. When we make such generalisations without using multiple measures, we are, in effect, making generalisations across measures for a given construct. 

It depend on how we operationalized our study; that is, how we defined the constructs and variables we wanted to measure, what methods  (i.e., interventions) we used for, and so forth. In my case the permission method itself is  static analysis.

The mono-method bias, the use of single method for evaluation, threatens the construct validity of the measurement procedure you use.

In my case, the correctness evaluation is done using multiple methods that reduces the threat to construct validity and external validity. Would the use of multiple methods have provided greater insight into the construct (correctness insight) than just a single method.

If the measurement procedure consists of a single method to assess the independent and/or dependent variables, this can act as a threat to construct validity. This is because the method used may introduce bias, changing the scores on the independent or dependent variable. In addition, the use of a single method becomes a threat to external validity because we may be making generalisations from our results that are really only accurate when using a specific type of method.

Experimenter bias becomes a threat to external validity because the results that are obtained in a given study may simply reflect the personal biases of the researcher. If another researcher were to carry out the same study using a sample with very similar characteristics and the same research methods, different results may be obtained. Therefore, our ability to generalise from the results of a study that is subject to experimenter bias is threatened. (in my case it is the manual correctness analysis).

\item Time and external validity
Time may defer by using different machine setup

\end{itemize}
\item[Internal Validity]
\end{description}



==> vitae.tex <==
\begin{itemize}
\item \textbf{Miss. Ayesha Sadiq} is a final year PhD student in the Faculty of Information Technology at Monash University. Her research interest primarily lies in software engineering with a focus on programming languages, program analysis and verification and formal modelling of real time applications.\\
\item \textbf{Dr. Yuan-Fang Li} is a Senior Lecturer at Faculty of Information Technology, Monash University, Australia. He received his PhD in computer science from National University of Singapore in 2006. His research interests include knowledge graphs, knowledge representation and reasoning, ontology languages, and software engineering.\\
\item \textbf{Dr. Sea Ling} works in the Faculty of Information Technology at Monash University as a senior lecturer. His fundamental research interest lies in software engineering techniques with specific focus on formal methods and programming languages.  Currently, his research is on extending and applying these techniques to the areas of ubiquitous and pervasive computing.
\item \textbf{Dr. Li Li} works in the Faculty of Information Technology at Monash University as ...
\end{itemize}

